An Abstraction-guided Approach to Scalable and Rigorous Floating-Point Error Analysis

Automated techniques for rigorous floating-point round-off error analysis are important in areas including formal verification of correctness and precision tuning. Existing tools and techniques, while providing tight bounds, fail to analyze expressions with more than a few hundred operators, thus unable to cover important practical problems. In this work, we present Satire, a new tool that sheds light on how scalability and bound-tightness can be attained through a combination of incremental analysis, abstraction, and judicious use of concrete and symbolic evaluation. Satire has handled problems exceeding 200K operators. We present Satire's underlying error analysis approach, information-theoretic abstraction heuristics, and a wide range of case studies, with evaluation covering FFT, Lorenz system of equations, and various PDE stencil types. Our results demonstrate the tightness of Satire's bounds, its acceptable runtime, and valuable insights provided.

==> NOT-NEEDED-background.tex <==

# <-- prevents compilation!!

A floating-point number systems, $\mathbb{F}$, is a subset of real numbers representable
in finite precision and expressed as a 5-tuple $(\beta, s, m, e, p)$.
Here, $\beta=2$ corresponds to the radix-2 floating-point system,
$p=53$ and $24$ for double and single precision numbers,
respectively, $s \in \{-1,1\}$ is the sign bit, $m$ is called the significand or
mantissa, and $e$ is the exponent. There are two types of floating-point
numbers, the {\em normals} and {\em denormals}, other than the special cases
of NaNs and infinities. Normal numbers lie in the interval
$[1, 2)$, while denormals are in $[0, 1)$.
%
%---For double-precision numbers, this range is $[-1022,1023]$. %$-1022 \leq e \leq 1023$.
%
Any such number, $\tilde{x} \in \mathbb{F}$ , has the value $s \cdot m \cdot \beta^e$.
%
If $x \in \mathbb{R}$, then $\tilde{x}$ denotes an element in $\mathbb{F}$
closest to $x$ obtained by applying the rounding operator($\circ$) to $x$.

The IEEE 754 standard defines four rounding modes for elementary floating-point
operations. Every real number $x$ lying in the range of $\mathbb{F}$ can be
approximated by a member $\tilde{x} \in \mathbb{F}$ with a relative error
no larger than the unit {\em round-off} $\bf{u}=\dfrac{1}{2}\beta^{1-p}$.
%
Here, $\beta^{1-p}$ represents the {\em unit of least precision (ulp)} for 
the exponent value of 1. Thus, to relate the quantities $\tilde{x}$ and $x$
over the rounding operator,
	if $x \in \mathbb{R}$ lies in the range of $\mathbb{F}$, then
$\tilde{x} = \circ(x) = x(1 + \delta),\quad |\delta| \leq \boldsymbol{u}.$\footnote{
 Later, we will employ $\delta_n$ to denote the $\delta$ applicable to the $n$th
 operator, etc.
}



Based on the radix and precision, the round-off quantity varies.
We support mixed-precision analysis, by suffixing the rounding
operator, when necessary, to denote the precision for the rounding. For example, when rounding
in double-precision we denote $\circ_{64}$.
%
Given two exactly represented floating-point numbers, $\tilde{x}$ and $\tilde{y}$,
arithmetic operators $\diamond in \{+,-,\cdot,/\}$ have the following guarantees:
\begin{equation}
\label{eq:opbound}
\begin{split}
	\circ(\tilde{x} \diamond \tilde{y}) &= (\tilde{x} \diamond \tilde{y})(1 + \delta),\quad |\delta| \leq \boldsymbol{u} \\
	&= (\tilde{x} \diamond \tilde{y}) + (\tilde{x} \diamond \tilde{y})\delta \\
	&= \{ \hbox{real value} \} + \{ \hbox{ round-off error } \}
\end{split}
\end{equation}

Thus, the rounded result involves an interval centered around the real exact value. The
width of this interval is determined by the amount of round-off error accumulated.

Besides the elementary operators, \satire supports other complex mathematical
operations such as transcendentals. In such cases, the bound on the $\delta$ terms changes
as a multiple of $\bf{u}$. We keep a default by configurable value for each operator,
allowing the user to obtain customized error bounds
for the specific math library being used.


During floating-point analysis, affine
arithmetic is employed to keep errors correlated.
%
In it, a quantity $\hat{x}$ is represented in affine form as
$\hat{x} = x_0 + \sum_{i=1}^n x_i \epsilon_i$,
where $x_0$ denotes the central value
and the $x_i$'s are finite floating-point numbers representing
noise coefficients
associated with the corresponding noise variables,
$\epsilon_i$'s. The $\epsilon_i$ are
formal variables whose value lies in $[-1,1]$
but are unknown until assigned. This representation
allows converging paths to cancel out error terms and improve
tightness.
%
For example $(x-x)$ in
affine analysis
will yield 0 because the noise variables can cancel
each other out.
Unlike affine analysis, interval analysis keeps widening the intervals.
%
\satire's approach can be viewed as ``symbolic affine''
(much like FPTaylor) in that
the noise coefficients,
$x_i$, are symbolic.


%--end





==> SAVED-illustrative-example.tex <==


\paragraph{\textbf{Illustrative example} : }In \satire, a straight line floating point code is parsed
into an abstract syntax tree(AST) where each node of the AST
corresponds to some mathematical operation. These
operations can be elementary operations like $\{+,-,\times,/\}$
or exponentials, transcendentals, etc. The number of incoming
paths defines the arity of that node. Prior to introducing the
formalism, we discuss here with a small example.
Figure ~\ref{fig:overview-illustration} shows the AST for the 
expression $S = (x\times(x+y)+z)\times 3.5$. Here, $x,y,z$ are the 
input variables with intervals $I(x), I(y)$ and $I(z)$ respectively.
In ~\cite{rosa,higham} the authors
introduce the decomposition of errors into {\em generated} round-off
errors and {\em propagation } of incoming errors.
We use  $E^{lr}$ to denote the local error term associated with a node.
The total error term for a node, denoted as $E^{tr}$, is then the additive 
composition of $E^{lr}$ and the propagation of the incoming error, $E^{prop}$.
 %--
\begin{figure}
	\centering
    \includegraphics[width=1.0\textwidth]{figs/overview-illustration.PNG}
  \caption{AST for $S = (x\times(x+y)+z)\times 3.5$, and the rebuilt AST with $v_2$ abstracted}
  \label{fig:overview-illustration}
\end{figure}
%--

In figure~\ref{fig:overview-illustration} each node defines a 2-tuple,
the first element being the symbolic expression,
and the second is the local error term. 
Nodes such as the `inputs' or the `abstracted' nodes have no dependence 
information available, that is, they cannot be unrolled further in the AST
hierarchy to more primitive nodes. For these nodes only the {\em total
error term} is stored.
%For nodes which do not have any 
%backward information stored, only the {\em total error term} is specified in
%the tuple, like in case of the input variables or the abstracted nodes. 
In the
figure we mark the nodes as a sequence of operations as in equation$~\eqref{eq:seqop}$
\begin{equation}
 \label{eq:seqop}
 v_1 = x+y;\quad v_2 = v_1\times x;\quad v_3 = v_2+z;\quad S = v \times 3.5
\end{equation}

Now consider the internal node $v_2$ for illustration of our analysis.
%
The sequence of computation on reaching the node $v_2$(with arity of 2) has two incoming components
--1) the operands in symbolic form, and 2) the incoming error terms also in symbolic form
from $v_1$ and $x$. Thus the total error term at $v_2$ is,
\begin{equation}
	\label{eq:internal-node-error}
  \begin{split}
  	E^{tr}(v_2) &= E^{lr}(v_2) + E^{prop}(v_2) \\
	            &= E^{lr}(v_2) + \bigg ( E^{tr}(x)\dfrac{\partial v_2}{\partial x} + E^{tr}(v_1)\dfrac{\partial v_2}{\partial v_1} \bigg ) =  E^{lr}(v_2) + \bigg ( E^{tr}(x)\cdot v_1 + E^{tr}(v_1)\cdot x \bigg )
  \end{split}
\end{equation}

Intuitively, the derivative term signifies the sensitivity of $v_2$ with respect to its
operands. Note that we have a total error term for $v_1$ in 
equation $~\eqref{eq:internal-node-error}$. It can be further unrolled into its local 
error forms and incoming dependencies as in equation $~\eqref{eq:v1-unroll}$

\begin{equation}
  \label{eq:v1-unroll}
  \begin{split}
  	E^{tr}(v_1) &= E^{lr}(v_1) + E^{prop}(v_1) \\
	            &= E^{lr}(v_1) + \bigg ( E^{tr}(x)\dfrac{\partial v_1}{\partial x} + E^{tr}(y)\dfrac{\partial v_1}{\partial y}\bigg ) = E^{lr}(v_1) + \bigg ( E^{tr}(x)\cdot 1 + E^{tr}(y)\cdot 1\bigg )
  \end{split}
\end{equation}

Plugging equation$~\eqref{eq:v1-unroll}$ into equation$~\eqref{eq:internal-node-error}$ 
gives us the total error for $v_2$ in terms of the local errors and incoming errors on
inputs.

\begin{equation}
\label{eq:v2-error-full}
   E^{tr}(v_2) = E^{lr}(v_2) + (2x+y)E^{lr}(x) + xE^{lr}(v_1) + xE^{tr}(y)
\end{equation}

The extent to which the error accumulated at $v_2$ impacts the output at $S$ depends
on the sensitivity of $S$ to changes in $v_2$, that is 
\[
	\dfrac{\partial S}{\partial v_2} = \dfrac{\partial S}{\partial v_3}\dfrac{\partial v_3}{\partial v_2} = 3.5
\]

Let $E^{tr}(S|v_2)$ denote the {\em total error component} at the output node, $S$, due to {\em total
error accumulated} at $v_2$, then
\begin{equation}
  \label{eq:v2-total-error-expr}
	E^{tr}(S|v_2) = E^{tr}(v_2) \dfrac{\partial S}{\partial v_2} = \bigg (E^{lr}(v_2) + (2x+y)E^{lr}(x) + xE^{lr}(v_1) + xE^{tr}(y)\bigg ) 3.5
\end{equation}

Equation$~\eqref{eq:v2-total-error-expr}$ is the symbolic form of the error contribution from $v_2$(and all its dependencies) to $S$, hence we need to maximize $E^{tr}(S|v_2)$ to obtain a bound on this contribution for which we invoke this expression on a global optimizer.

Few observations to note here,
\begin{compactitem}
  \item We obtain a function interval and an error interval by solving for $v_2$ and $E^{tr}(S|v_2)$ with the global optimizer. Note that $x,y$ and $v_1$ are of no more significance once we
  have solved for $E^{tr}(S|v_2)$ -- so $v_2$ can be abstracted as a free variable, $FV_2$, with 
  an associated error term and interval range as shown in the rhs of figure~\ref{fig:overview-illustration} resulting in a new and shortended AST. This abstraction technique allows us to incrementally solve for large depth expression graphs which otherwise become infeasible when building
 symbolic taylor-forms in one shot.
 \item In our example, abstracting node $v_2$ completely removed the dependency from $v_1$ and $x$, 
 hence was a good choice for abstraction. However, cinsider the case where $v_1$ is abstracted. 
 This would result in a loss of correlation between the reconvergent paths merging at $v_2$ for input $x$ 
 and running the risk of loosening the bounds especially when cancellations occur in the merging paths.
 However, our experiments show that with careful analysis to choose the abstraction depths guided by user
 adjustable knobs, \satire still obtains tight bounds as we will show in our evaluation study for `fdtd'.
 \item To find the total error at $v_2$ we unrolled its operand's error term, $E^{tr}(v_1)$ as well. Instead, if we only tracked the local error term at each node and scaled them by their respective propagation factors to the output, we end up with the same expression as in equation$~\eqref{eq:v2-local-error-only}$.
 %
 In contrast to existing tools, \satire identifies this balance in finding
 designated `cut' points where we can solve internal nodes for `total error' terms and abstract them removing their child dependencies . This process is repeated until the AST reaches a size that is easily managed using direct solve(unrolling all to local error terms) as illustrated in figure~\ref{fig:gradual-abstraction}.

\end{compactitem}

\begin{equation}
 \label{eq:v2-local-error-only}
 \begin{split}
 E^{tr}(S|v_2) &= \bigg (E^{lr}(v_2) + (2x+y)E^{lr}(x) + xE^{lr}(v_1) + xE^{tr}(y)\bigg )\dfrac{\partial S}{\partial v_2} \\
               &= E^{lr}(v_2)\dfrac{\partial S}{\partial v_2} + E^{tr}(x)\dfrac{\partial S}{\partial x} +
			      E^{lr}(v_1)\dfrac{\partial S}{\partial v_1} + 
				  E^{tr}(y)\dfrac{\partial S}{\partial y}
 \end{split}
\end{equation}


%We do this symbolically. A node in the AST is characterized
%by three symbolic quantities --1) its symbolic expression,
%2) its local error term, and 3) its sensitivity to the output
%obtained using symbolic algorithmic differentiation(AD).
%The advantage of doing symbolic AD makes it independent of specific input data values unlike
%ADAPT~\cite{adapt}.


\begin{comment}
A radix-2 floating point {\em normal} number (numbers whose
mantissae are of the form ``$1.m$'')
for a precision
$p$ (typically $p=32$, called single precision,
or $p=64$, called double precision) helps define a proper subset of
real numbers via a sign bit $s$, a mantissa word $m$ (23 bits
for single 52 for double) and an exponent word $e$ (8 bits for single
and 11 for double) via the formula $(-1)^s\cdot (1.m) \cdot 2^{e}$.
%
Subnormal numbers
are of the form $0.m$
and represent values below $2^{-126}$ (single) and below $2^{-1022}$ (double).
%
When rounding error is treated as ``noise''
and one performs a Taylor expansion, one is often concerned with
the {\em first-order error} which is what \satire estimates.
%
Second order error as well as subnormal values are of the same order,
are quite small, rarely matter,
and hence ignored in this work.\footnote{See
Section~\ref{sec:relwork} for discussions on where they don't matter
and where they do.}



IEEE754~\cite{ieee754} defines four 
rounding modes, of which we primarily consider {\em round to nearest}.
%
Define $\epsilon$ to be the {\em unit round-off} (the constant
$2^{-24}$ for single and $2^{-53}$ for double).
%
As per the first-order round-off error model, a calculation
such as $(x+y)$ introduces an error $(x+y) \epsilon$.\footnote
{We can be very specific about each operator's unit-roundoff: thus,
 $\epsilon_{+}$ would be more accurate.}
%
There is another concept called {\em unit in the last place} or $ulp$
whose magnitude is the least resolution at a particular value; in
particular, $ulp(1)=2\epsilon$, and doubles every binade (whenever the
exponent increases by 1). \skcmt{ulp definition is unclear. Can we use a more intuitive definition?}


In general, rounding errors are most serious when values
with very high exponent differences
are combined (e.g., added).
%
Often, a value with a very low exponent magnitude can disappear entirely.
%
Given that half of the representable floating-point numbers exist
in the interval $[-1,1]$,
there are many binades present in the interval $[0,1]$ and hence
for benchmarking examples, this forms a meaningful interval of inputs
to apply (and used in many of our examples).
%
If one wants to study benchmarks without much binade spread,
one can choose intervals such as $[1,2]$ within which
the values are apart by at most one binade. \skcmt{Is this what we do? If not, this is an odd proposition to put forth.}



\skcmt{Higher precision does not imply exact solution; so we could say ``get close to'' rather than obtain}
%
Given a floating-point expression,
one can obtain its ``true value'' (close to its real number value)
either by employing higher precision shadow value calculations
or libraries such as MPFR~\cite{mpfr}. 
%
The ``computed value'' is the one obtained after rounding
in the working precision.
%
{\em Absolute error} refers to the absolute difference between the
true and computed values, while
{\em relative error} is absolute error divided by the magnitude
of the true value.
%
Relative error provides a direct indication of the number of bits
lost due to rounding.\footnote{Unless the
true answer is close to $0$.}
%
In particular, for relative error $r$, the number of bits lost due
to rounding, $lost(r)$, equals $log_2(r/ulp(1))$.
%
This result captures the number of mantissa bits
necessary to represent the relative error
in terms of the number of $ulp(1)$ steps.


Given all this, it is possible to employ
\satire to estimate the maximum number of mantissa bits
lost (in support of precision profiling) as follows.
%
The answer produced by \satire is the estimated
absolute error.
%
Therefore,
if we manage to observe a value $v$ during an actual computation
and the \satire-estimated absolute error is $e$,
then one can take $v$ to be ``true value''
(as it happens to be observed in the real system)
and estimate the number of bits lost as $lost(e/v)$.
%
\skcmt{I don't get this argument. Above we say true value is exact, here we say true value is what us observed.}
%
We use these ideas in our results presented in
Section~\ref{sec:eval}.
\end{comment}

\begin{comment}
We now provide some insight into how
the symbolic Taylor Form approach works.
%
Consider the expression $(E_1+(E_1+E_2)$ where
$E_1$ and $E_2$ are complex 
%
The Symbolic Taylor Form approach
introduces ``noise'' variables at each operator
to model rounding.
%
%
In particular, the error-laden counterpart of 
$E_0 = x+(x+y)$ is modeled as
$E=(x+(x+y)(1+\epsilon_1))(1+\epsilon_2)$, where the magnitude of
$\epsilon_1$ and $\epsilon_2$ are bounded by $\epsilon$.
%
One can expand this expression using Taylor expansion
to reveal the first order error terms:
\( E = E_0
       + \epsilon_1 \cdot \frac{\partial E}{\partial \epsilon_1}
       + \epsilon_2 \cdot \frac{\partial E}{\partial \epsilon_2}
\)
%
Notice that $(E-E_0)$ is the absolute error.
%
Tools such as FPTaylor, Real2float, and Precisa rely on
{\em global optimizers} to compute the supremum of the
absolute error expression $(E-E_0)$.
%
%
Gelpia~\cite{fptaylor-toplas},
the global optimizer used in FPTaylor,
is based on
{\em interval branch and bound} (IBB~\cite{french-paper})
and relies on an efficient interval-arithmetic
solver~\cite{gaol} to estimate the bounds.


IBB tools rely on the key property of {\em interval
  monotonicity}:
for every operator $f$ used in the expression being
optimized, and for
intervals of real values $A$ and $B$ where
$A\subseteq B$, we must have $f(A)\subseteq f(B)$.
%
This monotonicity property
allows IBB-based tools to subdivide their input domains
and search over the population of subdivided domains.
%
Usually a heuristic (a genetic algorithm) guides the search,
and must be tuned with additional heuristics to properly
converge.
%
It is worth emphasizing that if this global optimization
process is not properly handled, two things can go wrong:
(1)~tight error bounds may not be obtained,
and
(2)~the optimization time can be enormous.
%
These are the points that \satire emphasizes.


It is worth observing from
$(E-E_0)$
that 

error anaysis on $E_1+(E_1+E_2)$,
one can either analyze this expression as such, or converted it
to $(E_1+E_1)+E_2$ and analyze---or even
convert it to $2E_1+E_2$ and analyze.
%
Are these choices equivalent?
%
Given that floating-point arithmetic does not obey
standard algebraic rules such as associativity,
the answer is ``no'' in general.
%
Floating-point arithmetic is also non-compositional.
%
For example, one can find input intervals for $x$
for which $(e^x-1)/x$ has {\em worse}
error than
$(e^x-1)/log_e(e^x)$~\cite{kahan}!


{\em More than the lack of associativity and lack of compositionality}, 
one must also keep in mind the ``quirky'' behavior of global
optimizers.
%
This problem is well-recognized in the global optimization
literature~\cite{cite-paper-benchmarking-global-opt}.
%
More specifically, for IBB-based global optimizers,
the answer is returned after a bounded number of steps
of search.
%
In this context,
it is important to keep
in mind that for examples with many suprema, it is important to
{\em canonicalize expressions before submitting to a global
optimizer}.
%
For example, if we submit $x*x$ for $x\in[-1,1]$ to Gelpia,
we find that it gives the answer $[-1,1]$ while if we feed
$x^2$, it returns $[0,1]$.
%
It is quite likely that $2E_1+E_2$ will return a far better
bound than
$E_1+(E_1+E_2)$  or
$(E_1+E_1)+E_2$.
%
In a nutshell,
  {\em \satire's tightness of bounds is critically dependent
  on these canonicalizations.}
%
Except for some rare corner cases of functions with many
local maxima/minima, canonicalizations almost always help,
and {\em is the key step to \satire's success with providing
  tight bounds, despite its scalability}.


(THIS CAN BE MOVED TO ANOTHER PLACE...)
\begin{sf}
  These correlations are so important in \satire that
we now highlight another situation where it is exploited.
%
When we add up the path contributions of errors at each backward
derivative application, we can either
do sum(abs(exps)) or abs(sum(exps)), and the latter is far better
as it canocalizes the term {\tt sum(exps)} to a significant extent.
%
If we were to do {\tt sum(abs(exps))}, we keep the exps apart
via the {\tt abs} function; they are ``insulated'' from each
other, resisting being combined.
%
Thus, while
sum(abs(exps)) and abs(sum(exps)) are real-equivalent, they
are not ``global optimizer equivalent.''
\end{sf}

 %--
\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{figs/introEx.pdf}
  \end{center}
  \caption{An Example Expression DAG}
  \label{fig:introEx-dag}
\end{wrapfigure}
%--


(ALSO TALK ABOUT reverse mode AD ideas with the help of the figure...)

The approach used in \satire is illustrated with the help of the
expression in Figure~\ref{fig:introEx-dag}.
%

Describe how the local error is generated at (y-x) and propagated
up the shown path via the reverse-mode AD.

Say we do an abstraction at *, we have x uncorrelated.

Stop with a solid connection between what we do in reverse-mode AD
and what FPTaylor does.


\end{comment}




==> SAVED-results-table.tex <==

\begin{table}[htbp]
\centering
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Benchmarks} & \multicolumn{2}{c}{Execution Time(seconds)} & \multicolumn{3}{c}{Absolute Error} & \multirow{2}{*}{\# operators}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} 
& {\satire} & {FPTaylor} & {\satire} & {FPTaylor} & {\satire (UnOpt)} &  \\
\midrule
exp1x				&		{\bf 0.083}	& 0.60			& {\bf 6.19E-14} 	& 2.04E-13  	& {\bf 6.19E-14}	&	5 	\\
exp1x\_32			&		{\bf 0.087}	& 0.42			& {\bf 9.71E-06}*	& 0.00010   	& {\bf 9.71E-06}	&	5 	\\
carbonGas			&		{\bf 0.084}	& 0.74			& {\bf 2.07E-08}	& 3.07E-08  	& {\bf 9.71E-06}	&	21	\\
x\_by\_xy			&		{\bf 0.068}	& 0.42			& {\bf 1.19E-07}	& 8.31E-07  	& {\bf 9.71E-06}	&	4 	\\
verhulst			&		{\bf 0.066}	& 0.47			&  4.27E-16			& {\bf 3.79E-16}& 4.47E-16			&	10	\\
turbine3			&		{\bf 0.154} & 0.49			&  3.58E-14			& {\bf 3.48E-14}& 4.10E-14		 	&	23	\\
turbine2			&		{\bf 0.102} & 0.49			& {\bf 6.32E-14}	& 7.36E-14  	& 7.39E-14			&	19	\\
turbine1			&		{\bf 0.097}	& 0.50			& {\bf 4.89E-14}	& 5.29E-14  	& 5.60E-14		 	&	24	\\
triangle			&		0.785       & {\bf 0.72} 	&  7.05E-14			& {\bf 4.06E-14}& 7.08E-14		 	&	14	\\
test05\_nonlin1\_test2&		{\bf 0.063}	& 0.40			& 1.11E-16			& 1.11E-16  	& 1.38E-16		 	&	4 	\\
test05\_nonlin1\_r4	&		{\bf 0.068}	& 0.41			& {\bf 1.11E-06}	& 2.78E-06 		& 1.94E-06			&	6 	\\
test02\_sum8		&		{\bf 0.080}	& 0.41			& 7.77E-15			& {\bf 7.11E-15}& 7.77E-15			&	15	\\
test01\_sum3		&		{\bf 0.125} & 0.40			& {\bf 1.13E-06}	& 1.97E-06  	& {\bf 1.13E-06}	&	11	\\
sum					&		{\bf 0.079}	& 0.40			& {\bf 3.44E-15}	& 3.66E-15 		& {\bf 1.13E-06}	&	11	\\
sqrt\_add			&		{\bf 0.072}	& 0.42			& {\bf 1.17E-15}	& 8.86E-15 		& 5.22E-15			&	7 	\\
sqroot				&		{\bf 0.074} & 0.46			&  8.82E-16			& {\bf 6.00E-16}& 8.82E-16			&	25	\\
sphere				&		{\bf 0.069}	& 0.42			& {\bf 8.88E-15}	& 1.03E-14  	& {\bf 8.88E-15}	&	9 	\\
sine				&		{\bf 0.122} & 0.50			&  7.36E-16			& {\bf 6.21E-16}& 7.36E-16			&	16	\\
sineOrder3			&		{\bf 0.065} & 0.44			&  1.09E-15			& {\bf 9.56E-16}& 1.09E-15		 	&	12	\\
sec4\_example		&		{\bf 0.085}	& 0.43			& {\bf 9.96E-10}	& 1.83E-09  	& 1.30E-09			&	8 	\\
rigidBody2			&		{\bf 0.084}	& 0.43			&  3.97E-11			& {\bf 3.61E-11}& 3.97E-11			&	17	\\
predatorPrey		&		{\bf 0.068}	& 0.48			& {\bf 1.73E-16}	& 1.74E-16  	& 1.75E-16			&	12	\\
nonlin2				&		{\bf 0.081}	& 0.43			& {\bf 9.96E-10}	& 1.83E-09  	& 1.30E-09			&	8 	\\
nonlin1				&		{\bf 0.072}	& 0.44			& {\bf 1.14E-13}*	& 4.37E-11  	& 2.92E-11			&	4 	\\
logexp				&		{\bf 0.062}	& 0.41			& {\bf 3.33E-13}	& 8.90E-13  	& 4.98E-13			&	5 	\\
jetEngine			&		1.969  		& {\bf 0.84}	& {\bf 2.88E-08}	& 7.09E-08  	& {\bf 2.88E-08}	&	35	\\
intro\_example		&		{\bf 0.069}	& 0.40			& {\bf 1.14E-13}*	& 4.37E-11  	& 2.92E-11			&	4 	\\
i4					&		{\bf 0.073}	& 0.41			& {\bf 3.53E-07}*	& 8.91E-06  	& {\bf 3.53E-07}	&	5 	\\
hypot32				&		{\bf 0.066} & 0.40			& {\bf 8.43E-06}*	& 0.00052  		& {\bf 8.43E-06}	&	6 	\\
himmilbeau			&		{\bf 0.090}	& 0.45			& {\bf 9.86E-13}	& 1.00E-12  	& {\bf 9.86E-13}	&	13	\\
exp1x\_log			&		{\bf 0.094}	& 0.43			&  2.39E-12			& {\bf 1.38E-12}& 3.09E-12			&	6 	\\
bspline3			&		{\bf 0.139} & 0.41			& {\bf 7.40E-17}	& 7.86E-17 		& {\bf 7.40E-17}	&	7 	\\
delta4				&		{\bf 0.119} & 0.45			&  1.26E-13			& {\bf 1.21E-13}& 1.26E-13			&	25	\\
delta				&		{\bf 0.416} & 0.53			& 3.30E-12			& {\bf 2.41E-12}& 3.30E-12			&	45	\\
doppler1			&		{\bf 0.158} & 0.58			&  1.49E-12			& {\bf 4.06E-13}& 1.71E-12			&	16	\\
doppler2			&		{\bf 0.164} & 0.59			&  2.98E-10			& {\bf 1.03E-12}*&3.55E-10			&	 16	\\
doppler3			&		{\bf 0.161} & 0.57			&  2.70E-13			& {\bf 1.60E-13}& 3.09E-13			&	16	\\
hypot				&		{\bf 0.068}	& 0.41			& {\bf 3.37E-13}	& 9.72E-13  	& 6.53E-13		 	&	6 	\\
kepler0				&		{\bf 0.094} & 0.43			& 1.10E-13			& {\bf 1.09E-13}& 1.10E-13			&	22	\\
kepler1				&		{\bf 0.168} & 0.46			&  7.07E-13			& {\bf 4.90E-13}& 7.07E-13			&	29	\\
kepler2				&		{\bf 0.402} & 0.52			&  3.20E-12			& {\bf 2.53E-12}& 3.20E-12			&	43	\\
rigidBody1			&		{\bf 0.076}	& 0.41			&  3.80E-13			& {\bf 2.95E-13}& 3.80E-13			&	12	\\
test04\_dqmom9		&		{\bf 0.206} & 0.63			& {\bf 9.66E-10}*	& 6.91E-05 		& 2.99E-05			&	35	\\
test06\_sums4\_sum1	&		{\bf 0.320} & 0.40			& {\bf 2.38E-07}	& 6.26E-07  	& {\bf 2.38E-07}	&	7 	\\
test06\_sums4\_sum2	&		{\bf 0.082}	& 0.40			& {\bf 2.38E-07}	& 6.26E-07 		& {\bf 2.38E-07}	&	7 	\\
\end{tabular}
\caption{Comparison of Results ({\bf bold-face} highlights better results, and * highlights
  a difference of more than an order of magnitude)}
	\label{table:satire-fptaylor}
\end{table}


==> abs.tex <==

  Rigorous and scalable floating-point error analysis is central to
  reasoning about and tuning numerical software.
  %  
  Today's analysis methods are unable to provide tight as well as
  rigorous guarantees even for straight-line expressions with
  about SMALLNUM expression DAG nodes.
  %
  In this paper, we provide a novel hybrid approach that synergistically combines
  multiple ideas to achieve this goal.
  %
  In particular, our work combines symbolic execution (to keep
  errors correlated similar to affine methods),
  backward derivatives (to suitably weigh errors flowing to the output),
  interval analysis (to allow users to explore input scenarios)
  and heuristically guided abstraction (to encapsulate a large amount of functionality
  without losing error correlation).
  %
  Our method implemented in a new tool Satern can handle very large expressions
  with BIGNUM expression DAG nodes.
  %
  We provide the new methodologies combined and
  our empirical studies that validate Satern's results on a number of
  real-world examples including several unraveled iterative loops including
  those that model systems of recurrences, stencils that
  model numerical computations, FFT, and scan.
  %
  We illustrate the insights provided by Satern for verification
  and end-uses such as precision tuning.
  %--
  


==> absguided.tex <==

% Here provide a diagram for the tool flow

% Then detail the abs-guided methodology, taking Lorenz as the running example

% Reasons for introducing the abstraction guided technique
Existing toolsets suffer from the drawback of
having to choose between the ability to provide tight guarantees 
or handle large expression sizes. 
%
FPTaylor, obtains tight bounds by building taylor forms
for the error expressions till the output node and the invoking
an optimizer..
%
While this is an extremely sound and accurate method enabling tight
bounds, building the taylor forms induces a significant cost
 as they begin to explode in size when stepping
beyond small expressions. This is because at every node an error
variable is introduced and its propagation is tracked in the forward 
path. Obtaining the full error expression is possible only after each error variable completes its traversal to the output node.
%
In the lorentz attractor example unrolled for just 10 iterations, 
FPtaylor times out after spending hours attempting to build
the taylor forms. It finishes building the taylor form for an unroll
of 5 iterations but produces a query so large that the optimizer 
cannot handle.
%
On the other hand, for industry scale application like
robotic controllers and avionic applications
where sounds guarantees are non-negotiable, enabling abstract interpretation often combined with interval or affine analysis allows faster reasoning on
the error bounds however trading off tightness of the bounds for scalability and soundness.

\satire's technique is motivated by the insight that the
techniques of abstraction and formulating symbolic error expressions
can be optimally combined to cultivate the best of both worlds obtaining tight bounds with the ability to handle large expression sizes.

\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figs/lorentz_second_var.png}
  \end{center}
  \caption{Single iteration DAG for updating second variable in lorentz attractor}
  \label{fig:expn-dag}
\end{wrapfigure}


To guarantee tightness of our bounds we enhance the notion of
separation and propagation of errors over symbolic expressions
and decouple the full error expression to be extracted at every internal node instead of being obtainable only at the output. 
%
This is enabled by introducing two passes, one forward and one backward.
\begin{compactitem}
  \item The forward pass associates an error generation term at every node it visits associated with the function expressions of that node.
  \item The backward pass enable reverse mode automatic differentiation
  to derive the symbolic propagation factors for each node.
  \item Thus we decompose an error expressions into its generative part obtained by the forward pass, and the propagation part obtain by the backward pass.
\end{compactitem}
%

  This technique enables decoupling the derivation of the error expression thus reducing  the overhead in obtaining the final expression enhancing the scalability to significantly large expressions sizes. For example, consider a discretized one dimensional heat equation
  unrolled over 10 steps comprising of 120 expression node. The complexity of these
  applications arises due to the structuring of the update process in stencils. 
  %
  Every node feeds into $M$ additional nodes in the forward path, where $M$ denotes the
  stencil's footprint, in this specific case a 3-point stencil.
  %

  FPtaylor takes close to 8hours generating the taylor forms and forming the final expression query for the global optimizer to work on. Furthermore, such a large optimization query pushes the optimizer signficantly in its attempts converge towards relevant bounds.
  Our technique can solve the unrolled heat equation in few seconds, in fact we handle much larger expressions. It is additionally guided by two heuristics. First being \satire's technique of decoupling the process of error expression formation, and secondly using best effort canonicalization for each individual expression query before feeding the optimizer.
  The helping optimizer involved for processing the final expression query involves
  an interval branch and bound algorithm(IBBA) aided with a genetic algoorithm based search
  technique. Interval based expression evaluations, although preety fast because of the 
  simplicity of the analysis involved, suffers from the detriment of loss of correlation.
  \{Expand some logic here, i just want to mention to preserve correlation\} Hence, 
  minimizing the number of individual occurences of each variable is essential for the
  search solution to converge quickly and tightly and make the best effort to avoid 
  being stuck in some local extrema. We utilize sympy/symengine's expression rewrite
  capabilities to obtain canonical representations of function expressions. The best 
  effort is to minimize the number of variable instances since multiple instances
  of the same variable will be treated as uncorrelated by interval solvers , hence
  requiring larger number of IBBA iterations to converge adequately. 
  %
  For example, in the example of the linear stencil solving the 
  heat equation, an efficient canonicalization would result in 
  each unique variable occuring only once in the final expression query.
  We should clarify here that this expression rewrite process is part of 
  generating the symbolic expression query and do not impact or change the
  original expression graph. The original expression graph structire is
  preserved unconditionally since floating point computation is non-compositional
  and hence changing computation order will impact the obtainable error bound.
  %
  With the best effort canonicalization process \satire can handle large expression
  graphs. We apply this technique to the `Finite Difference Time Domain" stencils used
  for solving Maxwell's equations. It involves 2 arrays representing the electric and
  magnetic field respectively and they update each other in every forward iteratio.
  For two arrays each of 500 domain points over 64 iterations amounts to around 192000
  computations being performed. That is an extremely large compute size for today's
  existing toolset. \satire solves this problem in around 2.5 hrs obtaining a tigh bound
  of 7.45e-13 when double precision rounding is turned on.

  \textbf{Now begin abstraction story.. this prelude was added to make the diff between linear and nonlinear expression canonicalization}

  Although canonicalization helps and is an important feature of \satire's
  process to help the optimizer queries, it can go only so far till it runs into
  problems with nonlinear and multivariate expressions. For linear expressions the rewrite
  process is fast and simple since it is primarily required to isolate and gather constant
  coefficients associated with different variables. However, when non-linear expressions
  are encouneted it becomes a best effort heuristic to isolate and simplify 
  nodes which can be combined  based on the order and degree of the instances.
  We revisit the lorentz attractor example to discuss such a scenario. 
  The lorentz attractor trces out a trajectory by solving a set of partial
  difference equation updating the next state $(x^\prime,y^\prime,z^\prime)$ based on its 
  current state of $(x,y,z)$. Below equations explain the guiding equations for
  one step of the iteration

	%% how to include split equations
  \begin{equation}
  \begin{split}
  	x^\prime &= (x + 10.0*(y - x)*0.005); \\
	y^\prime &= (y + (28.0*x - y - x*z)*0.005); \\
	z^\prime &= (z + (x*y - 2.666667*z)*0.005);
  \end{split}   
  \end{equation}

  If we simplify $y^\prime$, we obtain $(0.0 + 0.14*x + 0.995*y - 0.005*x*z)$. Note that the number of $y$ terms has reduced in this simple case. To make our case further, if we unroll once more iteration, the unsimplified and simplified form will be as shown in
  \begin{equation}
  \begin{split}
     unsim &= y + 0.005*(28.0*x - y - x*z) + 0.005*(-(x + 0.05*(-x + y))* \\
	       & (z + 0.005*(-2.666667*z + x*y)) + 28.0*(x + 0.05*(-x + y)) - \\
		   & (y + 0.005*(28.0*x - y - x*z))) \\
	 simp &= 0.0 + 0.2723*x + 0.997025*y - 1.25e-06*x*y**2 - 0.00966166665875*x*z \\
	      & - 2.375e-05*x**2*y - 0.00024666666625*y*z \\
  \end{split}
  \end{equation}

  Note that even though the simplified form is much smaller with unique occurences
  of each variable combination terms, these terms now begin to increase as a 
  multivariate polynomial due to the non-linearity of the expressions. Hence, even though
  canonicalization helps process larger queries, beyong a certain degree the best case
  heuristics reach a limit. We limit the expression synthesizing to be active between 8000
  to 30000 ops, since sympy has been seen to run into issues beyond that.
  
 % \adcmt{Cite and reason the limitations for sympy when handling large expressions.}
  To help push beyond this limit, we now introduce the concept of abstraction guided error analysis. The key motivation here is allowing the tool to solve for a set of internal nodes  which have significantly large expression graphs but not so large that our rewrite
  heuristics and optimizer queries are unable to handle. Once these internal nodes are solved for errors and a corresponding function interval, we abstract these nodes as free nodes. They become equivalent to an input node with an incoming error. Thus the mission to solve for the final output node restarts but now from a shallower depth since lots of the internal nodes have been abstracted. We do this iteratively at every few heuristically chosen depths as long as the expression op count remains within limits.

\begin{figure}
\centering 
\includegraphics[width=0.9\columnwidth]{figs/abstraction_fig.png}
\caption{Simple example showing the abstraction and related effects}
\label{fig:abstraction_fig}
%\vspace*{-1em}
\end{figure}

Figure ~\ref{fig:abstraction_fig} shows an example expression graph, part
of it being selected for abstraction and the post abstraction rearranged with the free variables and the change in depth of the expression. Here 
$f_i$ denotes the individual expression nodes and $x,y,z$ and $w$ are the input variables, as the formal notations already introduced. To further concretize the example, let us assign an actual
expression DAG as per the equations shown in equation $~\eqref{eq:abs-expr}$

\begin{equation}
	\label{eq:abs-expr}
\begin{split}
   f_6 &= y * z;\quad f_7 = \dfrac{f_6}{w} = \dfrac{(y*z)}{w}; \\
   f_5 &= x + f_6 = x + y*z;\quad f_3 = x * f_5 = x*(x+y*z); \\
   f_4 &= f_5 * f_7 = (x+y*z)*\dfrac{(y*z)}{w}; \\
   f_1 &= f_3 - f_4 = (x * f_5 = x*(x+y*z)) - ((x+y*z)*\dfrac{(y*z)}{w}); \\
   f_2 &= sin(f_4) = sin((x+y*z)*\dfrac{(y*z)}{w}); \\
   f_0 &= f_1 - f_2 = (x+y*z)*\dfrac{(y*z)}{w} - (x+y*z)*\dfrac{(y*z)}{w}; \\
\end{split}
\end{equation}

The total error at the output node $f_0$ per the notations introduced earlier will be
\begin{equation}
\label{eq:expr-sub1}
\begin{split}
  E^{tr}(f_0) = E^{lr}(f_0) 
              + E^{tr}(f_1)\dfrac{\partial f_0}{\partial f_1} 
			  + E^{tr}(f_2)\dfrac{\partial f_0}{\partial f_2}
\end{split}
\end{equation}

Equation $~\eqref{eq:expr-sub1}$ obtains the total error at the output node as the 
summation of the local error generated at $f_0$ with the total incoming error through
its operands $f_1$ and $f_2$. We can further unroll the total error terms of
$f_1$ and $f_2$ respectively as
\begin{equation}
\begin{split}
	E^{tr}(f_1) &= E^{lr}(f_1) 
	            + E^{tr}(f_3)\dfrac{\partial f_1}{\partial f_3} 
				+ E^{tr}(f_4)\dfrac{\partial f_1}{\partial f_4} \\
	E^{tr}(f_2) &= E^{lr}(f_2) 
				+ E^{tr}(f_4)\dfrac{\partial f_2}{\partial f_4} \\
\end{split}
\end{equation}

Plugging these back to the original error expression in $~\eqref{eq:expr-sub1}$ we obtain

\begin{equation}
\label{eq:full-expr}
\begin{split}
  E^{tr}(f_0) &= E^{lr}(f_0) + E^{lr}(f_1)\dfrac{\partial f_0}{\partial f_1} 
               + E^{lr}(f_2)\dfrac{\partial f_0}{\partial f_2} + 
			   + E^{tr}(f_3)\dfrac{\partial f_1}{\partial f_3}\dfrac{\partial f_0}{\partial f_1} \\
			  & + E^{tr}(f_4)\bigg ( \dfrac{\partial f_1}{\partial f_4}\dfrac{\partial f_0}{\partial f_1} 
			    + \dfrac{\partial f_2}{\partial f_4}\dfrac{\partial f_0}{\partial f_2} \bigg )
\end{split}
\end{equation}

The total error expression in equation $~\eqref{eq:full-expr}$ provides us
with two critical insights that form the core of the 
optimization strategies for \satire.
\begin{compactitem}
\item It indicates that if we keep unrolling the total error terms as per their children's dependencies, the final fully flattened expression will comprise of only local error terms emanating from each individual compute nodes scaled by the propagation factor. Thus the entire analysis can be factored into 
individual error expressions localized to each node, accumulated together at the end. This forms the primary decoupling tool that can evaluate the same
taylor forms albeit in a different compositional structure while avoiding
the taylor form expression size blow up encounetred by current tools.
\item Secondly, it suggests we can always choose to live in a world comprised
of a mixed set of local errors and total errors as in equation $~\eqref{eq:full-expr}$ which is equivalent to the original equation $~\eqref{eq:expr-sub1}$ and will also be equal to the expression obtained by complete unrolling. \end{compactitem}
Complete unrolling to only local error terms will still become huge 
for extremely large expressions like a 100K operations. 
Our \textbf{abstraction-guided} technique proposes this mixed methodology 
to obtain a balance between a full blown total error composition as done by
FPTaylor versus completely flattening out the expression to
local error terms. 

Let $get\_total\_error(node, abs)$ denote the function that takes 
the $node$ and abstraction option as an argument. Invoking
$get\_total\_error(f_0,abs=False)$ will unroll the whole error expression
in terms of symbolic local errors and generate a query to the optimizer
in terms of the primary inputs.
In our example of figure ~\ref{fig:abstraction_fig}, 
we enable abstraction by calling $get\_total\_error(f_0, abs=True)$.
Based on a best effort heuristic(we discuss later) suppose
it decides to unroll 
until reaching depth of 2, that is retaining the total error terms for nodes 
$f_5$ and $f_7$. The total error expression for $f_5$ and $f_7$ needs
to be obtained separately by further invoking
$get\_total\_error(f_5,abs=False)$ and $get\_total\_error(f_7,abs=False)$. 
The advantage we get by this abstraction is
if nodes selected for abstraction have large expression sizes and multiple
feed forward paths, it prevents the expression blow-up since we only 
propagate their concretized error value instead of the actual expressions.
  
Now $f_5$ and $f_7$ nodes can be casted as free nodes with no incoming dependencies but two associated attributes defining its total error and function
interval. Note that the actual inputs $y,z$ and $w$ can now be completely removed since they have already forwraded their contributions through $f5$ 
and $f_7$. However, we cannot remove the input $x$ since it has an existing contribution towards $f_3$. Thus, the new expression graph contains
three free variables in $x,f_5$ and $f_7$ with a shallower depth of 3. 

%% discuss heuristics next


==> absguided_bak.tex <==

% Here provide a diagram for the tool flow

% Then detail the abs-guided methodology, taking Lorenz as the running example

% Reasons for introducing the abstraction guided technique
Existing toolsets suffer from the drawback of
having to choose between the ability to provide tight guarantees 
or handle large expression sizes. 
%
FPTaylor, obtains tight bounds by building taylor forms
for the error expressions till the output node and the invoking
an optimizer..
%
While this is an extremely sound and accurate method enabling tight
bounds, building the taylor forms induces a significant cost
 as they begin to explode in size when stepping
beyond small expressions. This is because at every node an error
variable is introduced and its propagation is tracked in the forward 
path. Obtaining the full error expression is possible only after each error variable completes its traversal to the output node.
%
In the lorentz attractor example unrolled for just 10 iterations, 
FPtaylor times out after spending hours attempting to build
the taylor forms. It finishes building the taylor form for an unroll
of 5 iterations but produces a query so large that the optimizer 
cannot handle.
%
On the other hand, for industry scale application like
robotic controllers and avionic applications
where sounds guarantees are non-negotiable, enabling abstract interpretation often combined with interval or affine analysis allows faster reasoning on
the error bounds however trading off tightness of the bounds for scalability and soundness.

\satire's technique is motivated by the insight that the
techniques of abstraction and formulating symbolic error expressions
can be optimally combined to cultivate the best of both worlds obtaining tight bounds with the ability to handle large expression sizes.

\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figs/lorentz_second_var.png}
  \end{center}
  \caption{Single iteration DAG for updating second variable in lorentz attractor}
  \label{fig:expn-dag}
\end{wrapfigure}


To guarantee tightness of our bounds we enhance the notion of
separation and propagation of errors over symbolic expressions
and decouple the full error expression to be extracted at every internal node instead of being obtainable only at the output. 
%
This is enabled by introducing two passes, one forward and one backward.
\begin{compactitem}
  \item The forward pass associates an error generation term at every node it visits associated with the function expressions of that node.
  \item The backward pass enable reverse mode automatic differentiation
  to derive the symbolic propagation factors for each node.
  \item Thus we decompose an error expressions into its generative part obtained by the forward pass, and the propagation part obtain by the backward pass.
\end{compactitem}
%

  This technique enables decoupling the derivation of the error expression thus reducing  the overhead in obtaining the final expression enhancing the scalability to significantly large expressions sizes. For example, consider a discretized one dimensional heat equation
  unrolled over 10 steps comprising of 120 expression node. The complexity of these
  applications arises due to the structuring of the update process in stencils. 
  %
  Every node feeds into $M$ additional nodes in the forward path, where $M$ denotes the
  stencil's footprint, in this specific case a 3-point stencil.
  %

  FPtaylor takes close to 8hours generating the taylor forms and forming the final expression query for the global optimizer to work on. Furthermore, such a large optimization query pushes the optimizer signficantly in its attempts converge towards relevant bounds.
  Our technique can solve the unrolled heat equation in few seconds, in fact we handle much larger expressions. It is additionally guided by two heuristics. First being \satire's technique of decoupling the process of error expression formation, and secondly using best effort canonicalization for each individual expression query before feeding the optimizer.
  The helping optimizer involved for processing the final expression query involves
  an interval branch and bound algorithm(IBBA) aided with a genetic algoorithm based search
  technique. Interval based expression evaluations, although preety fast because of the 
  simplicity of the analysis involved, suffers from the detriment of loss of correlation.
  \{Expand some logic here, i just want to mention to preserve correlation\} Hence, 
  minimizing the number of individual occurences of each variable is essential for the
  search solution to converge quickly and tightly and make the best effort to avoid 
  being stuck in some local extrema. We utilize sympy/symengine's expression rewrite
  capabilities to obtain canonical representations of function expressions. The best 
  effort is to minimize the number of variable instances since multiple instances
  of the same variable will be treated as uncorrelated by interval solvers , hence
  requiring larger number of IBBA iterations to converge adequately. 
  %
  For example, in the example of the linear stencil solving the 
  heat equation, an efficient canonicalization would result in 
  each unique variable occuring only once in the final expression query.
  We should clarify here that this expression rewrite process is part of 
  generating the symbolic expression query and do not impact or change the
  original expression graph. The original expression graph structire is
  preserved unconditionally since floating point computation is non-compositional
  and hence changing computation order will impact the obtainable error bound.
  %
  With the best effort canonicalization process \satire can handle large expression
  graphs. We apply this technique to the `Finite Difference Time Domain" stencils used
  for solving Maxwell's equations. It involves 2 arrays representing the electric and
  magnetic field respectively and they update each other in every forward iteratio.
  For two arrays each of 500 domain points over 64 iterations amounts to around 192000
  computations being performed. That is an extremely large compute size for today's
  existing toolset. \satire solves this problem in around 2.5 hrs obtaining a tigh bound
  of 7.45e-13 when double precision rounding is turned on.

  \textbf{Now begin abstraction story.. this prelude was added to make the diff between linear and nonlinear expression canonicalization}

  Although canonicalization helps and is an important feature of \satire's
  process to help the optimizer queries, it can go only so far till it runs into
  problems with nonlinear and multivariate expressions. For linear expressions the rewrite
  process is fast and simple since it is primarily required to isolate and gather constant
  coefficients associated with different variables. However, when non-linear expressions
  are encouneted it becomes a best effort heuristic to isolate and simplify 
  nodes which can be combined  based on the order and degree of the instances.
  We revisit the lorentz attractor example to discuss such a scenario. 
  The lorentz attractor trces out a trajectory by solving a set of partial
  difference equation updating the next state $(x^\prime,y^\prime,z^\prime)$ based on its 
  current state of $(x,y,z)$. Below equations explain the guiding equations for
  one step of the iteration

	%% how to include split equations
  \begin{equation}
  \begin{split}
  	x^\prime &= (x + 10.0*(y - x)*0.005); \\
	y^\prime &= (y + (28.0*x - y - x*z)*0.005); \\
	z^\prime &= (z + (x*y - 2.666667*z)*0.005);
  \end{split}   
  \end{equation}

  If we simplify $y^\prime$, we obtain $(0.0 + 0.14*x + 0.995*y - 0.005*x*z)$. Note that the number of $y$ terms has reduced in this simple case. To make our case further, if we unroll once more iteration, the unsimplified and simplified form will be as shown in
  \begin{equation}
  \begin{split}
     unsim &= y + 0.005*(28.0*x - y - x*z) + 0.005*(-(x + 0.05*(-x + y))* \\
	       & (z + 0.005*(-2.666667*z + x*y)) + 28.0*(x + 0.05*(-x + y)) - \\
		   & (y + 0.005*(28.0*x - y - x*z))) \\
	 simp &= 0.0 + 0.2723*x + 0.997025*y - 1.25e-06*x*y**2 - 0.00966166665875*x*z \\
	      & - 2.375e-05*x**2*y - 0.00024666666625*y*z \\
  \end{split}
  \end{equation}

  Note that even though the simplified form is much smaller with unique occurences
  of each variable combination terms, these terms now begin to increase as a 
  multivariate polynomial due to the non-linearity of the expressions. Hence, even though
  canonicalization helps process larger queries, beyong a certain degree the best case
  heuristics reach a limit. We limit the expression synthesizing to be active between 8000
  to 30000 ops, since sympy has been seen to run into issues beyond that. 

  To help push beyond this limit, we now introduce the concept of abstraction 
  guided error analysis.
  %
  The key motivation here is allowing the tool to solve for a set of 
  internal nodes  which have significantly large expression graphs
  but not so large that our rewrite heuristics and optimizer queries
  are unable to handle. 
  %
  Once these internal nodes are solved for errors and a corresponding function interval,
  we abstract these nodes as free nodes.
  %
  They become equivalent to an input node with an incoming error.
  Thus the mission to solve for the final output node restarts but
  now from a shallower depth since lots of the internal nodes have
  been abstracted.
  %
  We do this iteratively at every few heuristically chosen depths 
  as long as the expression op count remains within limits.

\begin{figure}
\centering 
\includegraphics[width=0.9\columnwidth]{figs/abstraction_fig.png}
\caption{Simple example showing the abstraction and related effects}
\label{fig:abstraction_fig}
%\vspace*{-1em}
\end{figure}


  


==> arnab-analysis.tex <==

A finite numerical algorithm generates a sequence of computations,
\[
    s = (s_1, s_2, \dots, s_n)
\]

to obtain a final computed result, where $s_1$ are the primary inputs,
and $s_i$ being the result of the $i'th$ step is given by
\[
   s_i = \phi_i(s_1, s_2, \dots, s_{i-1})
\]

Here, $\phi_i$ is a mathematical opertaion or some computatble function
like transcendentals. This implies that the mathematical operation $\phi_i$
can involve as its inputs the primary inputs, $s_1$, and any of the
intermediary computed results leading upto the $i'th$ stage as its operands.

When such an algorithm is executed in finite precision, the operators $\phi_i$
are replaced by their floating point counterparts, that is,
\begin{equation}
\label{eq:intermediate-seq}
\begin{split}
	s_i^{fp} &= \phi_i^{fp}(s_1^{fp}, \dots, s_{i-1}^{fp}) \\
			 &= \phi_i^{fp}(s_1 + e_{s_1}, s_2 + e_{s_2}, \dots, s_{i-1} + e_{s_{i-1}}) \\
			 &= \phi_i(s_1 + e_{s_1}, s_2 + e_{s_2}, \dots, s_{i-1} + e_{s_{i-1}})( 1 + e_i) \\
\end{split}
\end{equation}

Here, $e_{s_j}$ represents the incoming error generated when computed $j'th$ step. The $e_i$ is
the rounding error generated in the $i'th$ step as the the floating point rounding model.

If $s_n$ is the final sequence of the compute, then one could write $s_n^{fp}$ as
%\begin{equation}
%\begin{split}
\[
  s_n^{fp} = \phi_n(s_1 + e_{s_1}, \dots, s_{n-1} + e_{s_{n-1}})( 1 + e_n) 
\]
 % 		   &= \phi_n(s_1 + e_{s_1}, \dots, s_{i-1} + e_{s_{n-1}}) +  \phi_n(s_1 + e_{s_1}, \dots, s_{i-1} + e_{s_{n-1}})e_n\\
%\end{split}
%\end{equation}

A taylor series expansion of the $\phi_n$ term on the rhs leads to the following

\begin{equation}
\begin{split}
  s_n^{fp} &= \bigg ( \phi_n(s_1, s_2, \dots, s_{n-1}) + \sum_{j=1}^{n-1} \dfrac{\partial s_n}{\partial s_j} e_{s_j} \bigg )( 1 + e_n) + O(e^2)\\
  &= \phi(s_1, \dots, s_{n-1}) +  \phi(s_1, \dots, s_{n-1})e_n + \sum_{j=1}^{n-1} \dfrac{\partial s_n}{\partial s_j} e_{s_j} + O(e^2) \\
  &= s_n + s_n\dot e_n + \sum_{j=1}^{n-1} \dfrac{\partial s_n}{\partial s_j} e_{s_j} + O(e^2)\\
\end{split}
\end{equation}

Here, $e_{s_n}$ is the total error, obtained at the final compute operation sequence of $s_n$. 
The max local error on at final stage is denoted as $E^{lr}(s_n) = \max(|s_n e_{n}|)$

Thus , the maximum total absolute error computed on the evaluation of the final term, $E^{tr}(s_n)$ is computed as

\begin{equation}
\begin{split}
  E^{tr}(s_n) &= |s_n - s_n^{fp}| = e_{s_n} = \leq \max(|s_n e_n| + |\sum_{j=1}^{n-1} \dfrac{\partial s_n}{\partial s_j} e_{s_j})| \\
  &\leq E^{lr}(s_n) + \max \bigg ( \sum_{j=1}^{n-1} |\dfrac{\partial s_n}{\partial s_j} E^{tr}(s_j))| \bigg )
\end{split}
\end{equation}



==> background-bak.tex <==


We provide background on floating-point arithmetic
emphasizing intuitions, and to better explain our results.
%
A radix-2 floating point {\em normal} number (numbers whose
mantissae are of the form ``$1.m$'')
for a precision
$p$ (typically $p=32$, called single precision,
or $p=64$, called double precision) helps define a proper subset of
real numbers via a sign bit $s$, a mantissa word $m$ (23 bits
for single 52 for double) and an exponent word $e$ (8 bits for single
and 11 for double) via the formula $(-1)^s\cdot (1.m) \cdot 2^{e}$.
%
Subnormal numbers
are of the form $0.m$
and represent values below $2^{-126}$ (single) and below $2^{-1022}$ (double).
%
When rounding error is treated as ``noise''
and one performs a Taylor expansion, one is often concerned with
the {\em first-order error} which is what \satire estimates.
%
Second order error as well as subnormal values are of the same order,
are quite small, rarely matter,
and hence ignored in this work.\footnote{See
Section~\ref{sec:relwork} for discussions on where they don't matter
and where they do.}



IEEE754~\cite{ieee754} defines four 
rounding modes, of which we primarily consider {\em round to nearest}.
%
Define $\epsilon$ to be the {\em unit round-off} (the constant
$2^{-24}$ for single and $2^{-53}$ for double).
%
As per the first-order round-off error model, a calculation
such as $(x+y)$ introduces an error $(x+y) \epsilon$.\footnote
{We can be very specific about each operator's unit-roundoff: thus,
 $\epsilon_{+}$ would be more accurate.}
%
There is another concept called {\em unit in the last place} or $ulp$
whose magnitude is the least resolution at a particular value; in
particular, $ulp(1)=2\epsilon$, and doubles every binade (whenever the
exponent increases by 1). \skcmt{ulp definition is unclear. Can we use a more intuitive definition?}


In general, rounding errors are most serious when values
with very high exponent differences
are combined (e.g., added).
%
Often, a value with a very low exponent magnitude can disappear entirely.
%
Given that half of the representable floating-point numbers exist
in the interval $[-1,1]$,
there are many binades present in the interval $[0,1]$ and hence
for benchmarking examples, this forms a meaningful interval of inputs
to apply (and used in many of our examples).
%
If one wants to study benchmarks without much binade spread,
one can choose intervals such as $[1,2]$ within which
the values are apart by at most one binade. \skcmt{Is this what we do? If not, this is an odd proposition to put forth.}



\skcmt{Higher precision does not imply exact solution; so we could say ``get close to'' rather than obtain}
%
Given a floating-point expression,
one can obtain its ``true value'' (close to its real number value)
either by employing higher precision shadow value calculations
or libraries such as MPFR~\cite{mpfr}. 
%
The ``computed value'' is the one obtained after rounding
in the working precision.
%
{\em Absolute error} refers to the absolute difference between the
true and computed values, while
{\em relative error} is absolute error divided by the magnitude
of the true value.
%
Relative error provides a direct indication of the number of bits
lost due to rounding.\footnote{Unless the
true answer is close to $0$.}
%
In particular, for relative error $r$, the number of bits lost due
to rounding, $lost(r)$, equals $log_2(r/ulp(1))$.
%
This result captures the number of mantissa bits
necessary to represent the relative error
in terms of the number of $ulp(1)$ steps.


Given all this, it is possible to employ
\satire to estimate the maximum number of mantissa bits
lost (in support of precision profiling) as follows.
%
The answer produced by \satire is the estimated
absolute error.
%
Therefore,
if we manage to observe a value $v$ during an actual computation
and the \satire-estimated absolute error is $e$,
then one can take $v$ to be ``true value''
(as it happens to be observed in the real system)
and estimate the number of bits lost as $lost(e/v)$.
%
\skcmt{I don't get this argument. Above we say true value is exact, here we say true value is what us observed.}
%
We use these ideas in our results presented in
Section~\ref{sec:eval}.


\begin{comment}
We now provide some insight into how
the symbolic Taylor Form approach works.
%
Consider the expression $(E_1+(E_1+E_2)$ where
$E_1$ and $E_2$ are complex 
%
The Symbolic Taylor Form approach
introduces ``noise'' variables at each operator
to model rounding.
%
%
In particular, the error-laden counterpart of 
$E_0 = x+(x+y)$ is modeled as
$E=(x+(x+y)(1+\epsilon_1))(1+\epsilon_2)$, where the magnitude of
$\epsilon_1$ and $\epsilon_2$ are bounded by $\epsilon$.
%
One can expand this expression using Taylor expansion
to reveal the first order error terms:
\( E = E_0
       + \epsilon_1 \cdot \frac{\partial E}{\partial \epsilon_1}
       + \epsilon_2 \cdot \frac{\partial E}{\partial \epsilon_2}
\)
%
Notice that $(E-E_0)$ is the absolute error.
%
Tools such as FPTaylor, Real2float, and Precisa rely on
{\em global optimizers} to compute the supremum of the
absolute error expression $(E-E_0)$.
%
%
Gelpia~\cite{fptaylor-toplas},
the global optimizer used in FPTaylor,
is based on
{\em interval branch and bound} (IBB~\cite{french-paper})
and relies on an efficient interval-arithmetic
solver~\cite{gaol} to estimate the bounds.


IBB tools rely on the key property of {\em interval
  monotonicity}:
for every operator $f$ used in the expression being
optimized, and for
intervals of real values $A$ and $B$ where
$A\subseteq B$, we must have $f(A)\subseteq f(B)$.
%
This monotonicity property
allows IBB-based tools to subdivide their input domains
and search over the population of subdivided domains.
%
Usually a heuristic (a genetic algorithm) guides the search,
and must be tuned with additional heuristics to properly
converge.
%
It is worth emphasizing that if this global optimization
process is not properly handled, two things can go wrong:
(1)~tight error bounds may not be obtained,
and
(2)~the optimization time can be enormous.
%
These are the points that \satire emphasizes.


It is worth observing from
$(E-E_0)$
that 

error anaysis on $E_1+(E_1+E_2)$,
one can either analyze this expression as such, or converted it
to $(E_1+E_1)+E_2$ and analyze---or even
convert it to $2E_1+E_2$ and analyze.
%
Are these choices equivalent?
%
Given that floating-point arithmetic does not obey
standard algebraic rules such as associativity,
the answer is ``no'' in general.
%
Floating-point arithmetic is also non-compositional.
%
For example, one can find input intervals for $x$
for which $(e^x-1)/x$ has {\em worse}
error than
$(e^x-1)/log_e(e^x)$~\cite{kahan}!


{\em More than the lack of associativity and lack of compositionality}, 
one must also keep in mind the ``quirky'' behavior of global
optimizers.
%
This problem is well-recognized in the global optimization
literature~\cite{cite-paper-benchmarking-global-opt}.
%
More specifically, for IBB-based global optimizers,
the answer is returned after a bounded number of steps
of search.
%
In this context,
it is important to keep
in mind that for examples with many suprema, it is important to
{\em canonicalize expressions before submitting to a global
optimizer}.
%
For example, if we submit $x*x$ for $x\in[-1,1]$ to Gelpia,
we find that it gives the answer $[-1,1]$ while if we feed
$x^2$, it returns $[0,1]$.
%
It is quite likely that $2E_1+E_2$ will return a far better
bound than
$E_1+(E_1+E_2)$  or
$(E_1+E_1)+E_2$.
%
In a nutshell,
  {\em \satire's tightness of bounds is critically dependent
  on these canonicalizations.}
%
Except for some rare corner cases of functions with many
local maxima/minima, canonicalizations almost always help,
and {\em is the key step to \satire's success with providing
  tight bounds, despite its scalability}.


(THIS CAN BE MOVED TO ANOTHER PLACE...)
\begin{sf}
  These correlations are so important in \satire that
we now highlight another situation where it is exploited.
%
When we add up the path contributions of errors at each backward
derivative application, we can either
do sum(abs(exps)) or abs(sum(exps)), and the latter is far better
as it canocalizes the term {\tt sum(exps)} to a significant extent.
%
If we were to do {\tt sum(abs(exps))}, we keep the exps apart
via the {\tt abs} function; they are ``insulated'' from each
other, resisting being combined.
%
Thus, while
sum(abs(exps)) and abs(sum(exps)) are real-equivalent, they
are not ``global optimizer equivalent.''
\end{sf}

 %--
\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{figs/introEx.pdf}
  \end{center}
  \caption{An Example Expression DAG}
  \label{fig:introEx-dag}
\end{wrapfigure}
%--


(ALSO TALK ABOUT reverse mode AD ideas with the help of the figure...)

The approach used in \satire is illustrated with the help of the
expression in Figure~\ref{fig:introEx-dag}.
%

Describe how the local error is generated at (y-x) and propagated
up the shown path via the reverse-mode AD.

Say we do an abstraction at *, we have x uncorrelated.

Stop with a solid connection between what we do in reverse-mode AD
and what FPTaylor does.


\end{comment}




==> eval-bak.tex <==

% eval

We evaluate \satire on an extensive set of benchmarks.
Firstly we perform a comparative study of \satire's performance 
with FPTaylor on FPTaylor's reported benchmarks. These benchmarks
are currently part of the FPBench community ranging over a wide 
variety of applications including polynomials approximations,
non-linear expressions, expressions from control theory, logarithmic benchmarks and from biological modeling. Additionally, we introduce an
exhaustive set of fresh benchmarks for evaluating \satire
that contains large expression sizes obtained by unrolling large domain
problems from partial differential equations ranging over
solving heat equations, maxwell's equations , tracing trajectory
using lorentz attractor. We also introduce error analysis on prefix sums
and techniques to analyze FFT by partioniing the complex evalution
into real and imaginary datapaths separately. 
Furthermore, we perform empirical evaluations on randomply 
generated input data bounded by the test input intervals
to show the tightness of the bounds. Additionaly, we perform
relative error profiling on these benchmarks to showcase
actual loss of precision bits at runtime.

\paragraph{Experimental Setup\ :}
\satire is compatible with python3. The internal
symbolic engine is powered by the sympy and symengine modules.
All benchmarks were executed with Python3.8.0 version on a
dual 14-core Intel Xeon CPU E5-2680v4 2.60GHz CPUs system(total
28 processor cores) with 126 GB of RAM. The comparative data
for FPTaylor were generated on the same machine configuration.

\subsection{\textbf{Comparative Study}}



\begin{table}[htbp]
\centering
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Benchmarks} & \multicolumn{2}{c}{Execution Time(seconds)} & \multicolumn{2}{c}{Absolute Error} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} 
& {\satire} & {FPTaylor} & {\satire} & {FPTaylor} \\
\midrule
exp1x				&		0.083	& 0.60	& 6.19E-14		& 2.04E-13 \\
exp1x\_32			&		0.087	& 0.42	& 9.71E-06		& 0.00010 \\
carbonGas			&		0.084	& 0.74	& 2.07E-08		& 3.07E-08 \\
x\_by\_xy			&		0.068	& 0.42	& 1.19E-07		& 8.31E-07 \\
verhulst			&		0.066	& 0.47	& 4.27E-16		& 3.79E-16 \\
turbine3			&		0.154   & 0.49	& 3.58E-14		& 3.48E-14 \\
turbine2			&		0.102   & 0.49	& 6.32E-14		& 7.36E-14 \\
turbine1			&		0.097	& 0.50	& 4.89E-14		& 5.29E-14 \\
triangle			&		0.785   & 0.72	& 7.05E-14		& 4.06E-14 \\
test05\_nonlin1\_test2&		0.063	& 0.40	& 1.11E-16		& 1.11E-16 \\
test05\_nonlin1\_r4	&		0.068	& 0.41	& 1.11E-06		& 2.78E-06 \\
test02\_sum8		&		0.080	& 0.41	& 7.77E-15		& 7.11E-15 \\
test01\_sum3		&		0.125   & 0.40	& 1.13E-06		& 1.97E-06 \\
sum					&		0.079	& 0.40	& 3.44E-15		& 3.66E-15 \\
sqrt\_add			&		0.072	& 0.42	& 1.17E-15		& 8.86E-15 \\
sqroot				&		0.074   & 0.46	& 8.82E-16		& 6.00E-16 \\
sphere				&		0.069	& 0.42	& 8.88E-15		& 1.03E-14 \\
sine				&		0.122   & 0.50	& 7.36E-16		& 6.21E-16 \\
sineOrder3			&		0.065   & 0.44	& 1.09E-15		& 9.56E-16 \\
sec4\_example		&		0.085	& 0.43	& 9.96E-10		& 1.83E-09 \\
rigidBody2			&		0.084	& 0.43	& 3.97E-11		& 3.61E-11 \\
predatorPrey		&		0.068	& 0.48	& 1.73E-16		& 1.74E-16 \\
nonlin2				&		0.081	& 0.43	& 9.96E-10		& 1.83E-09 \\
nonlin1				&		0.072	& 0.44	& 1.14E-13		& 4.37E-11 \\
logexp				&		0.062	& 0.41	& 3.33E-13		& 8.90E-13 \\
jetEngine			&		1.969   & 0.84	& 2.88E-08		& 7.09E-08 \\
intro\_example		&		0.069	& 0.40	& 1.14E-13		& 4.37E-11 \\
i4					&		0.073	& 0.41	& 3.53E-07		& 8.91E-06 \\
hypot32				&		0.066   & 0.40	& 8.43E-06		& 0.00052 \\
himmilbeau			&		0.090	& 0.45	& 9.86E-13		& 1.00E-12 \\
exp1x\_log			&		0.094	& 0.43	& 2.39E-12		& 1.38E-12 \\
bspline3			&		0.139   & 0.41	& 7.40E-17		& 7.86E-17 \\
delta4				&		0.119   & 0.45	& 1.26E-13		& 1.21E-13 \\
delta				&		0.416   & 0.53	& 3.30E-12		& 2.41E-12 \\
doppler1			&		0.158   & 0.58	& 1.49E-12		& 4.06E-13 \\
doppler2			&		0.164   & 0.59	& 2.98E-10		& 1.03E-12 \\
doppler3			&		0.161   & 0.57	& 2.70E-13		& 1.60E-13 \\
hypot				&		0.068	& 0.41	& 3.37E-13		& 9.72E-13 \\
kepler0				&		0.094   & 0.43	& 1.10E-13		& 1.09E-13 \\
kepler1				&		0.168   & 0.46	& 7.07E-13		& 4.90E-13 \\
kepler2				&		0.402   & 0.52	& 3.20E-12		& 2.53E-12 \\
rigidBody1			&		0.076	& 0.41	& 3.80E-13		& 2.95E-13 \\
test04\_dqmom9		&		0.206   & 0.63	& 9.66E-10		& 0.99928 \\
test06\_sums4\_sum1	&		0.320   & 0.40	& 2.38E-07		& 6.26E-07 \\
test06\_sums4\_sum2	&		0.082	& 0.40	& 2.38E-07		& 6.26E-07 \\
\end{tabular}
	\label{table:satire-fptaylor}
\end{table}

Table ~\ref{tab:satire-fptaylor} presents the comparative results between
\satire and FPTaylor. While \satire excels in its ability to handle large
and complex expressions, we show through this comparative study that even
for smaller benchmark suites it obtains comparable and in many cases tighter bounds than today's state of the
error analysis tools, albeit comparing with FPTaylor. 
%
Comparison is presented for both the total execution times and the absolute
error bounds over a suite of 47 benchmarks exported from FPTaylor's supported
suite. 
%
In all of the listed benchmarks both \satire and FPTaylor
generated extremely tight bounds within the same orders of magnitude.
Furthermore, \satire obtains even slightly tighter bounds in over 50\% of these
benchmarks while providing an average 4.5 times speed-up in execution times.
%
Deeper analysis of the cases where we observe a significant improvement
in the error bound obtained by \satire is primarily attributed
to its simplification feature. Consider the case for the `Direct Quadrature
Moments Method'(dqmom) benchmark. \{Briefly add with reference what dqmom does\}
%
FPTaylor reports an error bound of 6.909e-05 with its real function interval range in
[-9.0e+10, 9.0e+10]. \satire obtains an extremely tight bound
for dqmom with an absolute error bound of 9.66e-10 with its real function interval range
in [-9.0e+05, 9.0e+05]. We performs over 10k random simulations on the input
interval ranges and find that thr empirical error seen when compared with a 
high precision shadow value evaluation of this benchmark always satisfies
\satire's significantly tighter bound. Satire is able to extract this tightness of
bounds by performing simplifications on the final error expressions in symbolic form
before feeding into the optimizer. These simplification procedures are concerned with
making a best effort attempt to keep single instances of an input multi or single variate term
wherever possible by expanding the expression in a polynomial form and rearranging similar
occuring terms together. In interval analysis, multiple occurences of the same variable fails
to preserve any correlation between these terms leading to exploding the resulting intervals.
Since our optimizer is an Interval Branch and Bound Analysis(IBBA), it is subject to the same
difficulties with correlation. Thus applying the simplification procedure and canonicalizing
expressions attempts to reduce the occurence of the same variable instances which in turn reduces the 
loss of correlation leading to tighter bounds as seen in the dqmom example.
%
To support our hypothesis, we extract the Taylor forms generated by FPTaylor for dqmom and post-processed
it through our simplification framework before to the optimizer. We observe that such a simplified taylor
form generates significantly tighter bound of 9.62e-10 post simplification with a result comparable to \satire's
prediction.
%
This analysis brings afore a key insight that obtaining tight bounds for error analysis is primarily dependent 
on two factors -- (1) firstly, the methodology employed to obtain the symbolic error expressions, be it as
a taylor form expansion as in FPTyalor, or symbolic generate and propagate technique as in \satire, (2) and 
secondly, how efficiently the final error expression is processed when passing it through an optimizer
or an iterative non linear SMT solver \{cite rosa \}. The second point highlights the differences one may see when attempts 
are made to fine tune these expressions with knowledge of the solvers solving them in the backend which
may significantly influence the resulting bounds as evident in the dqmom example.


\subsection{\textbf{Analysis on Larger Benchmarks}}

\satire's primary advantage in error analysis of floating point expressions is
in its ability to scale to large expression sizes at a scale no other current
toolset currently operates. We achieve this performance capability due to
two key attributes in \satire's design -- 1) Decoupling the full error expression
into individual generate and propagate components \{cite Rosa \} thus reducing
the toll of carrying around a large expression impacting memory bandwith,
2) Introducing guided abstraction, that allows incrementally solving the total error
terms locally at internal nodes and abstracting them with constant error terms instead of
the symbolic expressions. Here, we analyze multiple large scale benchmarks and how each
of these technques helps and impacts the obtained bounds.

\paragraph{Stencils: } Stencils belong to an important class of 
iterative solvers operating on dense arrays modeling partial
difference equations with applications ranging from 
fluid dynamics, cosmology, combustion, etc. 
%
They form essential building blocks for solving
larger more composite problems and as such knowledge 
of the accumulated round-of errors are of importance 
for ensuring overall correctness.
%
However, these comprise of
large and dense arrays being updated over time and
involving spatial dependencies between the grid points
as shown in figure ~\ref{fig:iteratedStencil} for a 3-point stencil.
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figs/iteratedStencil.png}
  \end{center}
  \caption{Iterative structure of a 3 point stencil}
  \label{fig:iteratedStencil}
\end{wrapfigure}

There are 2 key features presents in such computational update schemes
which makes obtaining a tight and rigorous error bound critical. 
%
Firstly, each point in this system contributes to a set of
neighbouring points in the immediate future
as per the arity of the stencil.
%
Thus, an error term(round-off or otherwise)
generated locally at a certain grid point will effectively 
spread across the compute space as the simulation progresses.
%
Secondly, there are many interconnected contributing terms emanating from 
a point that merge in the forward path. It implies preserving correlations
when forming error expression is essential for such computations.
%
This is because pure interval analysis will move the needle towards 
widening error intervals due to the spatial spread of
contributions. However, preserving correlations symbolically or
using affine analysis will bring back correlations for tighter bounds.
Even so, obtaining a quantifiable error bound in such applications becomes 
important atleast over few iterations of the application which allows the 
developers a level of confidence in its numerics.
%

Absence of tools to provide rigorous bounds for such applications forces developers to
resort to empirically validating the numerics using shadow value computations
or rely on statistically obtained precision qualities, neither of which are 
provavbly rigorous.
%
When applied to existing tools , they are faced with the difficuly in handling
such interconnected computational structures even for few iterations. For example,
solving for a one dimensional heat stencil formed by unrolling the stencil structure of figure ~\ref{fig:iteratedStencil}  for only 
10 iterations requires FPTaylor executing for almost 8 hours to complete its
symbolic taylor form building stage. Inherently this means we cannot apply
such rigorous tools for any practical cases of these examples required to
iterate over atleast 100 of iterations and even more-so for multidimenisonal cases 
of these problems.
%

\satire can solve the above stencil benchmark comprising of around 400 operations
within 4 seconds obtaining an absolute error bound of 6.10e-15. Unrolling this
stencil for 32 iterations results in 4226 compute nodes and requires a solving
time of 170 seconds with an absolute error bound o 1.95e-14.

%% add a result without partial solve

\subsection{\textbf{Empirical Evaluation}}         

\subsection{\textbf{Relative error profiles}}




==> formal.tex <==

\subsection{Formal Details of \satire}
% formal
%--
\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{figs/cavfig.png}
  \end{center}
  \caption{A Generic Expression DAG}
  \label{fig:expn-dag}
\end{wrapfigure}
%--
In this section, we will introduce the notations necessary to define
expression DAGs and how we can conduct forward symbolic execution
as well as backward derivatives for error estimation.
%
We present a generic expression DAG
in Figure~\ref{fig:expn-dag} for the expression

\[ E = f_0(f_1(f_2(x_5, f_3(x_2)), x_4), f_4(x_4, f_5(x_1, x_3)), f_5(x_1, x_3))\]


%
Given an expression $E$ over input variables $X=\{x_1,\ldots,x_m\}$
that are associated with intervals of input values $I=\{\iota_1,\ldots,\iota_m\}$,
and with outputs $Y=\{y_1,\ldots,y_n\}$,
our goal is to obtain the first-order error at these outputs.
%
Let $f$ be a function symbol (``operator'') appearing somewhere in
the given expression DAG (e.g., $f_0, f_4$, etc).
%
Let $f^{1}$ be the operator of the first child of $f$ (e.g.,
$f^{2}_4 = f_5$).
%
Generalizing this notation, 
let $f^{ijk}$ denote the $k$th child of the $j$th child of the
$i$th child of $f$ (thus $f^{112}_0 = f_3$), and
in general we will use $f^{\sigma}$ to denote the
node located starting at $f$ and following the path specified
by the sequence of positive non-zero integers $\sigma$.
%
Let $Exp(f)$ stand for the {\em expression} denoted
by the $f$ node
(e.g., $Exp(f_0) = E$ and $Exp(f_2) = f_2(x_5,f_3(x_2))$).
%
By $Exp(f^i)$ we mean the $i$th argument {\em expression} of $f$.
(e.g., $Exp(f^3_0) =  f_5(x_1,x_3)$).
%
We will use the notation $Exp(f^{ijk})$ to denote the
expression denoted by the $f^{ijk}$ node
(e.g., $Exp(f^{112}_0) =  Exp(f^3) = f_3(x_2)$)
and we will use $Exp(f^{\sigma})$ to locate the expression
at node $f^{\sigma}$.



The total rounding error at the output of an operator $f$
is denoted by $Err^{t}(f)$ and can be
overapproximated by adding the local rounding error
generated by $f$, denoted by $Err^{l}(f)$, and the ``amplified
incoming error'' propagaged by $f$.
%
The local rounding error at the output of an expression is
overapproximated by the value produced at the output of the
expression {\em times} the unit roundoff value $\epsilon$ introduced
earlier.
%
The ``amplification factor'' for this error is nothing but the backward partial derivative.
%
Thus,
\[ E^{tr}(f_0)  = E^{lr}(f_0)
            + E^{tr}(f_1) \cdot \frac{\partial f^{e}_0}{\partial f^{e}_1}
            + E^{tr}(f_4) \cdot \frac{\partial f^{e}_0}{\partial f^{e}_4}
            + E^{tr}(f_5) \cdot \frac{\partial f^{e}_0}{\partial f^{e}_5}             
\]
%
To define $E^{tr}(f_1)$, $E^{tr}(f_4)$, and $E^{tr}(f_5)$, we will need to recurse down the paths
below these operators.
%
We will use the notation $E^{tr}(f^{\sigma})$ to index ``down the path'' from $f$ following
the path $\sigma$ and refer to the total error at $f^{\sigma}$.
%
Then we can pick up the total rounding error generated by node $f^{\sigma}$ and amplify it
as needed.
%
To simplify exposition,
let us denote this amplification factor by {\em path strength};
thus $ps(f,f^{\sigma})$ is how much the total round-off at node $f^{\sigma}$ gets amplified
when traversing up the $\sigma$ path toward $f$.
%
This notation then allows us to write
%
\[ E^{tr}(f) = E^{lr}(f) + E^{tr_{\sigma}}(f) \cdot ps(f,f^{\sigma}). \]
%
Let the notation $n:\sigma$ denote the
$\sigma$ sequence extended by ``consing''
$n$ at the head (e.g.,
let $"345"$ be the sequence consisting of $3$, $4$, and $5$; then $2:"345"$
= $"2345"$).
%
Using this notation, we now define $ps$ inductively as follows:
%
\begin{itemize}
\item \( ps(f,f^n) = \frac{\partial f^{e}}{\partial f^{e_n}} \)
\item \( ps(f,f^{n:\sigma}) = \frac{\partial f^{e}}{\partial f^{e_n}} \cdot
                           \frac{\partial f^{e_n}}{\partial f^{e_{\sigma}}} 
\)
\end{itemize}
%
Now, as far as our example goes,
our goal is to define the errors at the outputs $y_1$ and $y_2$.
%
These are nothing but
the errors at $E^{tr}(f_1)$ and $E^{tr}(f_0)$, respectively.
%
We will illustrate the calculation of the latter in detail (the former is similar).
%
The error $E^{tr}(f_0)$ is nothing but the addition of
$E^{lr}(f_0)$ and the errors incoming to operator $f_0$ from ``below''.
%
We basically need to add up the incoming errors across all paths that flow into $f$.
%
More formally,
%
\[ E^{tr}(f) = E^{lr}(f) + (\sum_{\sigma} E^{tr_{\sigma}}(f) \cdot ps(f,f^{\sigma})). \]
%
As an illustration,
$E^{tr}(f_0)$ is obtained by adding
to $E^{lr}(f_0)$ the errors coming into $f_0$ from all the operators reachable
below $f_0$ via {\em all} descending paths.
%
When the paths are of maximal length, they touch an input, and then the local rounding
error is $0$ (e.g., in Figure~\ref{fig:expn-dag}, we denote the local rounding error generated
by nodes $x_1$ through $x_5$ as being $0$).
%
Notice that the paths $\sigma$ must include paths of length $1$, $2$, $\ldots$, $M$
where $M$ is the maximum depth of the expression DAG.
%
In our example, we will sum over the following example paths $\sigma$:
$"1"$, $"2"$, $"3"$, $"1"$, $"11"$, $"111"$, $"21"$, $"221"$, $\ldots$,
$"32"$.


\subsection{How the Formalism is Realized in \satire}

{\bf INFORMAL WRITING; POLISH LATER}

In \satire, there is an upward sweep where symbolic expressions are built while
parsing, and during a ``downsweep'', we carry out the indicated summation.
%
More formally, the $e$s are calculated level by level using a sliding window
within which a cost function is evaluated.
%
The AST size grows linearly while the op-count is a function of the reconvergence
and can even be exp.
%
There are ways to keep unfolded equations as a substitution list to contain
size growths (as in linear unification) but to obtain the benefits of


%

to get canonicalization benefits, we keep substituting out and get

more common subexpressions

%%
%


==> ganesh-analysis.tex <==




% formal
%--
\begin{figure}
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figs/formalization-fig.pdf}
  \end{center}
  \caption{A Generic Expression DAG, and Modeling Error Flows}
  \label{fig:expn-dag}
\end{figure}
%--
In this section,\ggcmtside{This section tries to unify all notations. Once this is debugged, use it everywhere!}
we introduce our notations for
expression DAGs as well as error analysis.
%
A problem instance in \satire is given as a tuple $(E, X, I, Y)$
where $E$ is the expression to be analyzed---e.g.,
Figure~\ref{fig:expn-dag} capturing the expression.
%
\[ E = f_0(f_1(f_2(x_5, f_3(x_2)), x_4), f_4(x_4, f_5(x_1, x_3)), f_5(x_1, x_3))\]
%
Here, $X=\{x_1,\ldots,x_m\}$ are the input variables each confined
to intervals of {\em floating-point} values $I=\{\iota_1,\ldots,\iota_m\}$,
and the goal is to tightly estimate the output intervals
at outputs $Y=\{y_1,\ldots,y_n\}$ in terms of floating-point
values.\ggcmtside{Make sure outputs are also FP...}


Let $f$ be a function symbol (``operator'') appearing somewhere in
the given expression DAG (e.g., $f_0, f_4$, etc).
%
Let $f^{\#}$ denote the arity of $f$ (e.g., $f_0^{\#} = 3$).
%
Let $f^{1}$ be the operator of the first child of $f$ (e.g., $f^{2}_4 = f_5$).
%
Generalizing this notation, 
let $f^{ijk}$ denote the $k$th child of the $j$th child of the
$i$th child of $f$ (e.g., $f^{112}_0 = f_3$).
%
For a sequence of positive non-zero integers $\sigma$ (e.g., $112$
in the above example),
let $f^{\sigma}$ denote the
node located starting at $f$ and following the path specification $\sigma$.
%
Let ${\cal E}(f)$ stand for the {\em expression} whose
principal operator $f$ is (e.g.,
${\cal E}(f_2) = f_2(x_5, f_3(x_2))$).
%
Let ${\cal E}(f^i)$ denote the expression whose principal operator
$f^i$ is (e.g., ${\cal E}(f^3_0) =  f_5(x_1,x_3)$).
%
We can naturally generalize this to uniquely identify subexpressions
anywhere in the DAG using ${\cal E}(f^{\sigma})$.


\paragraph{Error Analysis:\/}
At every operator site $f$,
let $\hat{{\cal E}}(f)$ denote the IEEE-rounded result of ${\cal E}(f)$,
which is \( \hat{{\cal E}}(f) = {\cal E}(f) (1+e_f) \) where
$e_f$ is the range within which the rounding error of $f$ falls:
from \S\ref{sec:background}, we know this to be $\epsilon_f$ in magnitude.
%
We use the ``hat'' to denote errors flowing out
(the purple output arrow in Figure~\ref{fig:expn-dag}'s inset).
%
Clearly, there is error (``from below'') flowing into each operator, and 
we model the effect of these errors taken separately by
the notation $ \check{{\cal E}}(f) $
(the violet incoming arrows in Figure~\ref{fig:expn-dag}'s inset causing
 the violet output).
 %
 Building on this notation,
 let us use the notation $ \overline{{\cal E}}(f) $
 to denote the output of ${\cal E}(f)$ under the presence
 of both these error flows
(the black outgoing arrow in Figure~\ref{fig:expn-dag}'s inset).


%
We can model $ \check{{\cal E}}(f) $ through first-order Taylor analysis and arrive at
%
\[  \check{{\cal E}}(f) = {\cal E}(f) +
%
    \sum_{i=1}^{f^{\#}}  {\overline{\cal E}(f^i) } \cdot \frac { \partial {\cal E}(f) } { \partial {\cal E}(f^{i}) }
%
    \]
    %
    where the partial derivative models the change in $ {\cal E}(f) $
    for a unit change in $ {\cal E}(f^i) $.
    %

    We can now define $ \overline{\cal E}(f) $ as follows:
    %
\[  \overline{{\cal E}}(f) = (1+e_f)\cdot ( {\cal E}(f) +
      \sum_{i=1}^{f^{\#}}  {\overline{\cal E}(f^i) } \cdot
      \frac { \partial {\cal E}(f) } { \partial {\cal E}(f^{i}) }
   )
%
      \]

      We assume that
      all the error magnitudes
      ($\hat{{\cal E}}(f)$,
       $\overline{{\cal E}}(f)$, and
      $\check{{\cal E}}(f)$)
      are of the order of $\epsilon_f$, and their products are ignored
      during second-order analysis.
      %      
      Applying this simplification, we get

      \[  \overline{{\cal E}}(f) =
          {\cal E}(f) +
          {\cal E}(f) \cdot e_f +
          \sum_{i=1}^{f^{\#}}
              {\overline{\cal E}(f^i) }
              \cdot
              \frac { \partial {\cal E}(f) } { \partial {\cal E}(f^{i}) }
%
      \]      
      and so, the magnitude of $ \overline{{\cal E}}(f) - {\cal E}(f)$ is
      bounded from above by
      \[
          {\cal E}(f) \cdot \epsilon_f +
          \sum_{i=1}^{f^{\#}}
              {\overline{\cal E}(f^i) }
              \cdot
              \frac { \partial {\cal E}(f) } { \partial {\cal E}(f^{i}) }
              \]
              Denote by $ps(f,f^i)$ the {\em path strength}: how much does ${\cal E}(f)$
              ``wiggle'' for a unit-wiggle of ${\cal E}(f^i)$.
              %
              We can generalize this to
              $ps(f,f^{\sigma})$\footnote{Exactly as ``backprop'' in reverse-mode AD in SGD does.}
%              
              This allows
              us to  upper bound of the error at the output of $f$ by
      \[
          {\cal E}(f) \cdot \epsilon_f +
          \sum_{i=1}^{f^{\#}}
              {\overline{\cal E}(f^i) }
              \cdot
              ps(f,f^i)
              \]
              %
              
              \noindent In general, {\em the contribution of error at $f$'s output} by an
              operator situated deep-down in the DAG, say $f^{\sigma}$, 
              can be  upper-bounded by
      \[
          {\cal E}(f) \cdot \epsilon_f +
          \sum_{i=1}^{f^{\#}}
              {\overline{\cal E}(f^{\sigma}) }
              \cdot
              ps(f,f^{\sigma})
              \]

              \noindent              If we take the view that we
              have no a priori knowledge of how errors cancel,
              then {\em the total error at the output of $f$} as contributed
              by {\em all the operators in the DAG} can be expressed as
              upper-bounded by
              %
              \[ \overline{\cal E}(f) = \hat{\cal E}(f) +
              (\sum_{\sigma} \overline{{\cal E}}(f^{\sigma}) \cdot ps(f,f^{\sigma}))\;\; . \]

              \noindent A crucial observation capitalized in \satire is that
              error-correlations are realized in the process of {\em canonicalization}.
              %
              More specifically, here is how \satire works:
              %
              \begin{compactitem}
              \item The expression DAG is built during forward symbolic execution where
                the step of canonicalization {\em coalesces} common subexpressions as
                much as possible, thus bringing in error correlations.\footnote{If
                  the abstraction criterion for complexity reductions is met, then
                  the ``black-box'' so created will not further canonicalize with respect
                  to later forward symbolic execution steps.}
                
              \item The path-strength products are applied as in the above
                equation\ggcmtside{Number it and refer to it...}
                {\em incrementally}.
                %
                After each of the
                products $ \overline{{\cal E}}(f^{\sigma}) \cdot ps(f,f^{\sigma}) $
                we
                \begin{compactitem}
                \item Add the symbolic expressions.\ggcmtside{Here talk about the abs sum versus
                  sum of abs etc.} This is a {\bf hugely} important step that realizes further
                  canonicalizations.
                \item Once fully canonicalized, we evaluate the expressions with
                  respect to the intervals in $I$, thus obtaining the error bounds
                  in $Y$.
                \end{compactitem}
              \end{compactitem}
              
              
              
    



==> ganesh-intro.tex <==
Numerical software systems modeling scientific and engineering applications
heavily rely on floating-point arithmetic.
%
The round-off errors that build up in these systems at run time
are a major correctness concern.
%
In the past, critical applications ranging from statistical
computing and econometric software~\cite{economic,numstats} to weapon
systems~\cite{patriot-missile} have failed due to these errors.
%
There is also growing pressure to employ reduced-precision arithmetic,
as doing so can save on energy consumption and improve performance.
%
Unfortunately, this can make round-off error accumulation even worse. 


In order to ensure the safety of systems in the presence of rounding
and generate rigorous correctness guarantees, tools that provide
rigorous bounds on output roundoff error for given intervals of
inputs are crucial.
%
A number of such tools have been developed, including
Fluctuat~\cite{fluctuat}, Gappa~\cite{gappa},
PRECiSA~\cite{precisa}, Real2Float~\cite{real2float},
Rosa~\cite{rosa}, FPTaylor~\cite{DBLP:journals/toplas/SolovyevBBJRG19},
Numerors~\cite{DBLP:conf/sas/JacqueminPV18}, 
and tools specialzed for cyberphysical systems \cite{munoz-winding,rocco-solver-nfm-2019}.
%
Analysis for reduced precision can be readily supported by such tools
(e.g., \cite{fptuner}).


%Floating-point arithmetic is widely employed across many scientific
%and engineering applications.
%%
%Rigorous analysis of the round-off error introduced by floating-point
%operations is important in many contexts.
%%
%Those interested in {\em verification}
%typically focus on rigorously bounding the round-off error to be within 
%chosen limits (an important step in verifying
% many hardware/software systems~\cite{darulova-cps}
% and cyberphysical systems~\cite{titolo-munoz-winding-number}).
%%
%Those focused on {\em tuning} typically combine
% different implementations (e.g., single
% and double precision computations)
% of floating-point functions to achieve
% an overall implementation that achieves given round-off error targets
% while reducing the overall computational cost
% (important for improving
%  energy consumption and performance~\cite{some-other-rigorous-tuning,fptuner,precimonious}).
%%
%Another application is
% {\em precision profiling} in which
% one tries to estimate the relevant number of 
% mantissa bits as a computation proceeds.
%%
%Precision profiling methods
%(e.g., \cite{verificarlo,verrou}) allow one to understand
%opportunities for changing the working precision.



Unfortunately, even the best of today's {\em rigorous} and
{\em automated} round-off error
bounding tools can handle expressions with no more than a few hundred
operators~\cite{fptaylor,fpbench}.
%~\cite{toplas-paper-tool-citations,fpbench-examples}.
%
Unfortunately, expressions of thousands of operators
are commonplace in almost all practical situations:
recurrence equation solving schemes ~\cite{lorentz},
the Fast Fourier Transform (FFT) algorithm, and other familiar
algorithms such as parallel prefix sum (scan) 
or partial differential equation (PDE) solving
stencil algorithms.
%
To tackle such sizes rigorously,
abstract interpretation and/or
theorem-proving methods~\cite{fluctuat,munoz-winding,munoz-gappa,boldo-2nd-order-wave}
must be employed; this entails manual effort.
%~\cite{fluctuat,winding-number,more-refs,munoz-gappa-pvs,boldo-2nd-order-wave}
%
The other is to shed rigorous guarantees and
settle for sampling based
methods~\cite{sc13-precimonious,hifptuner,herbie,craft,adapt}
or Monte-carlo methods~\cite{verificarlo,stoke-fp}
that bound error based on 
the observed error on randomly selected input points.
%
Scalability alone is insufficient: {\em tight} overapproximations
are important.



In this work, we introduce a scalable and rigorous approach
for error analysis embedded in a new tool
\satire({\bf S}calable
{\bf A}bstraction-guided {\bf T}echnique for {\bf Incremental} {\bf R}igorous
analysis of round-off {\bf E}rrors) that offers scalability as well
as rigorous and tighter error estimates than all tools in its class.
%
In this paper, we thorougly explain \satire's algorithms providing insights on
its overall performance, and also provide extensive benchmarking studies
that cover two aspects: (1)~sensitivity studies that explain the effects of the different
algorithmic choices on \satire's result quality and scalability, and (2)~scaling
studies that give an indication of the sizes of problems that can be
handled using \satire.




%% Introduce Satire here ... then in following text build contardictions with 
%% Satire for every new pointers of discussion


Traditionally, error analysis has been conducted
using interval analysis, which provides efficient approaches to
obtain error bounds.
%
It is well-known that interval analysis, while rigorous,
provides loose error bounds, as it
inherently looses correlation
between variables,
resulting in quite pessimistic bounds.
%
While affine analysis maintains these correlations,
the bounds can get quite pessimistic as well, especially for
non-linear expressions such as $x/(x+1)$.
%
The recently proposed method of rigorously computing
{\em Symbolic Taylor Forms} and embodied in the
FPTaylor tool~\cite{toplas}
avoids both these problems associated with interval
and affine methods.
%
Moreover, as reported in~\cite{DBLP:journals/toplas/SolovyevBBJRG19,DBLP:conf/sas/JacqueminPV18},
FPTaylor also produces some of the tightest bounds across
a spectrum of benchmarks
when compared against existing tools.
%
However FPTaylor does not handle the scale of
expression sizes that arise even in small benchmarks.
%
For example, for the discretized one dimensional heat flow
(``1D-heat'') equation
calculation using a stencil whose temporal application
is unrolled over 10 time steps, about 442 operators are
generated.
%
FPTaylor takes about 8 hours simply to generate the Taylor form,
following which
the global optimizer that comes with FPTaylor gives up.
%

In contrast, \satire handles the aforesaid 1D-heat problem
in a few seconds.
%
\satire also has handled expressis with over 200K operators
drawn from realistic examples.
%
In addition, \satire\ generates tighter error bounds than
FPTaylor on most of FPTaylor's examples (details in Section~\ref{sec:eval}).


To give an early indication on the kinds of results we are
able to obtain using \satire, we provide in
Table~\ref{tab:small-comparison} a sampling of examples
and our results obtained using \satire and FPTaylor
(a much more comprehensive evaluation is provided in Section~\ref{sec:eval}).
%
Like all the other tools in its
class (e.g., \cite{gappa,precisa,real2float,rosa,DBLP:conf/sas/JacqueminPV18})
\satire also works with straight line
floating point code with support for mixed precision analysis and multi-output
estimation with improved scalability. 

%% -- adding a small comparative table early on --
\begin{table}[htbp]
\centering
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Benchmarks} & \multirow{2}{*}{\# operators} & \multicolumn{2}{c}{Exec Time (secs)} & \multicolumn{2}{c}{Absolute Error} &
\raisebox{-4ex}{\shortstack[l]{Empirical Max\\ Abs Error}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & {\satire} & {FPTaylor} & {\satire} & {FPTaylor} \\
\midrule
jetEngine 			& 35 	& 1.969   & {\bf 0.84}	& {\bf 2.88E-08}	& 7.09E-08 & 1.57e-12\\
kepler2	  			& 43 	& {\bf 0.402}   & 0.52	&  3.20E-12		& {\bf 2.53E-12} & 3.49e-13\\
dqmom	  			& 35 	& {\bf 0.206}   & 0.63	& {\bf 9.66E-10}* & 6.909e-05  & 3.27e-13 \\
heat1d-10steps		& 442 	& {\bf 2.1} & - & 6.1062e-15 & NA & 5.45e-16 \\
FFT-1024pt 			& 43k 	& {\bf 180} & - & 7.80e-13 & NA & 6.18e-15\\
Lorentz-20steps		& 307 	& {\bf 284} & - & 1.25e-14 & NA & 3.59e-15 \\
fdtd1d-64steps		& 192k & {\bf 9711} & - & 7.45e-13 & NA & 9.89e-16\\
\end{tabular}
\label{tab:small-comparison}
\end{table}
%%

The benchmarks 
of jetengine, kepler and dqmom are from FPTaylor's suite of relatively
large operator counts.
%
The heat-flow, FFT, Lorentz Contraction (non linear) and FDTD (finite-difference
time-domain, used in hundreds of areas including electromagnetic simulation) are added as part of
\satire's benchmarks to show its performance for even larger operator counts.
%
These large numerical kernels used in scientific computing provide insights
into \satire's capabilities.
%
The last column of the table shows the empiricaly seen
(using shadow-value calculations at a higher precision)
maximum absolute error over
10k simulations of each of these kernels for randomly
distributed data points in the specified interval.
%
For the kernels where
a comparable bound from FPTaylor is unavailable, the emprirical bound
statistically shows the tightness of \satire's bounds.


\paragraph{Contributions:} \satire makes the following contributions:
\begin{compactitem}
\item \satire
      supports the ability to
      create abstractions of large
      subexpressions
      during forward symbolic evaluation
      (explained in Section~\ref{sec:absguided})
      based on user-specified cost metrics.
      %
      Section~\ref{sec:eval} shows that the error estimates
      following abstraction
      are still quite informative (not grossly exaggerated)
      in most cases.      
      We will illustrate abstractions with the help      
      of Figure~\ref{fig:gradual-abstraction} momentarily.
         %
         Abstractions are key to \satire's scalability.

\item Most important of all,
      \satire   performs error calculations
      {\em incrementally}
      while walking the expression
      graph---instead of the monolithic approach taken in
      tools such as FPTaylor.
      %
      This incremental approach is another key
      contributor to \satire's scalability.

\item \satire combines interval analysis and symbolic analysis to
      achieve a good
      tradeoff between scalability and correlation of errors.

\item \satire performs
      {\em canonicalization} of expressions during symbolic
      analysis that allows
      its back-end global optimizer to convergence to
      tight error bounds.
      %
      The effectiveness of canonicalization was confirmed
      by applying this step to the Symbolic Taylor Forms
      produced by FPTaylor whereupon
      the error bounds became tighter
      (we discuss this in Section~\ref{sec:eval}).

\end{compactitem}


\subsection{Illustration of Abstractions}
\label{sec:key-contribs}


%--
\begin{figure}
	\centering
    \includegraphics[width=1.0\textwidth]{figs/gradual-abstraction-illustration.PNG}
  \caption{Incremental error analysis using gradual abstraction}
  \label{fig:gradual-abstraction}
\end{figure}
%--


\subsubsection{Abstractions}

\satire improves scalability by introducing a notion of
{\em node abstraction } that helps guide the  
forward error analysis in incremental steps.%
Figure~\ref{fig:gradual-abstraction} illustrates the incremental solving scheme using
abstraction.
%
It shows an iterative stencil's evolution in time .
%
Two successive abstractions are performed followed by a direct compute for the
final output error.
%
Intuitively, \satire builds symbolic error expressions
feeding into a global optimizer for obtaining the maximum error.
To counter the explosion of the symbolic expressions for large AST
depths and interconnected networks, 
it allows for partitioning the AST using a cost
metric guided heuristic and user knobs to abstract the compute nodes
at such designated `cut' points. These selected nodes are solved in isolation
for their errors and the AST is rebuilt with these nodes as free variables
with an in-flowing error term. Our results
in Section~\ref{sec:eval} show that \satire can handle a variety
of problems
of very large expression sizes and also produces tight guarantees.


Thus, \satire can
serve as a stand-alone error-bound verifier for large expressions,
or be used as a primitive tool within a theorem-proving context
(when it may help reduce the number of proof-decomposition
      steps).
%      
It can also help in the the roles of
rigorous precision profiling
and provide precision tuning.




\satire's design takes advantage of the best of many
existing approaches, and adds its own set of unique directions:

%--

\subsection{Canonicalizations}

Our methodological contributions are now 

Our key contribution is that of 

Consider the case for `dqmom' where \satire's bounds are much tighter
than the previously reported FPTaylor bounds.

Multiple occurences of the same variable looses correlation
when treated with `interval based' optimizers.
\satire stresses on {\em simplifying
symbolic expressions} to reduce the individual occurence of a variable
term. We call this process as {\em canonicalization} or {\em simplification}.
Feeding the optimizer with this synthesized expressions optimized
for preserving correlation(through canonicalization)
aids better convergence results for \satire.





FPTaylor
on most of the benchmarks analyzed by FPTaylor.




\noindent{\bf Roadmap:\/}

ROADMAP of the paper

\begin{comment}

% intro

Any formal activity involving floating-point expressions---be it formal
verification, rigorous precision tuning, or some other---centrally relies
on our ability to provide {\em tight} error bounds for {\em large}
expressions.
%
Unfortunately, even the best of today's methods suffer from the following
drawbacks: (1)~they can provide tight bounds, but for small expressions
using methods such as affine analysis combined with symbolic (SMT)
reasoning~\cite{eva,others,dont-forget-thomas-wahl},
Taylor forms~\cite{taylor-forms},
or other methods~\cite{other-methods};
(2)~they can provide loose bounds for larger expressions, either using
interval-based methods~\cite{some-intvl-methods}, empirical (sampling)
methods~\cite{all-sampling-based-prec-analysis-such-as-in-sc19-tut}, or
statistical methods such as Monte-carlo arithmetic~\cite{mca}.
%
There are {\em no available} methods that handle multi-output expressions
involving, for instance, 4,000 inputs and 
involve expression DAGs with a maximum depth of hundreds.
%
These are the kinds of expressions one can obtain in many practical
situations.
%
Some of the situations that give rise to such expressions include:
%
\begin{compactitem}
\item Unraveled arithmetic computations such as
  parallel prefix sums (scan), stencil-based computations for
  solving partial differential equations (PDE) or optimized implementations
  algorithms of central importance such as FFT.

\item Recurrences that model the solutions of equations based on Newton's
  method~\cite{newton} or
  standard benchmarks with highly unstable trajectories such
  as Lorenz attractors~\cite{lorenz}.
\end{compactitem}
%
Unfortunately, today's precision analysis methods simply cannot deal
with these sort of expressions unless they heavily employ (unsound)
underapproximations that often rely on shadow-value calculations
on a limited number of input points, or highly useless bounds obtained through
interval branch-and-bound search algorithms.
%
This prevents recent advances in floating-point reasoning and tuning from
handling sizes that practitioners would care.


  In this paper, we provide a novel hybrid approach that synergistically combines
  multiple ideas to achieve this goal.
  %
  In particular, our work combines the best features of
  many methods including symbolic execution,
  automatic differentiation,
  interval analysis, 
  and guided abstraction.
  %
  Our method implemented in a new tool Satern can handle very large expressions
  with BIGNUM expression DAG nodes.
  %--
  Such results are being obtained in the area of formal analysis of floating-point
  arithmetic for the first time.


  (Say more.)
  
\end{comment}







==> intro-bak.tex <==
Floating-point arithmetic underlies many critical
scientific and engineering applications.
%
Round-off errors introduced during floating-point
%
computations have resulted in egregious errors
in applications ranging from statistical
computing and econometric software~\cite{economic,numstats} to critical
defense systems~\cite{patriot-failure}.
%
To guard against such errors, formal verification tools are essential, and
a basic capability in such tools is the ability to
{\em rigorously} estimate the round-off error generated by
floating-point expressions for given input intervals.
%
This capability is also important in designing
rigorous mixed-precision tuning systems
(e.g., \cite{fptuner}).


A number of tools for rigorous round-off analysis have been
developed: Fluctuat~\cite{fluctuat}, Gappa~\cite{gappa},
PRECiSA~\cite{precisa}, Real2Float~\cite{MagronCD15},
Rosa~\cite{rosa}, FPTaylor~\cite{DBLP:journals/toplas/SolovyevBBJRG19},
Numerors~\cite{DBLP:conf/sas/JacqueminPV18}, 
and tools specialized for cyberphysical systems
\cite{munoz-winding,rocco-solver-nfm-2019} to name a few.
%
Unfortunately, these tools
cannot {\em automatically} handle floating-point
expressions of thousands of operators
that arise in even the simplest of practical situations
including recurrence equation solving schemes and
algorithms such as the Fast Fourier Transform (FFT) and %, and other familiar
%algorithms such as
parallel prefix sum.
%
Today's tools in this space
can at best handle expressions with a few dozen operators.
%
To tackle large sizes automatically, one must today employ
abstract interpretation methods and/or
theorem-proving
methods~\cite{fluctuat,munoz-winding,munoz-gappa,boldo-2nd-order-wave}.
%
The use of non-rigorous
approaches that employ concrete evaluation on a reasonable sampling
of the input space~\cite{sc13-precimonious,hifptuner,herbie,craft,adapt}
or Monte-Carlo-style approached~\cite{verificarlo,stoke-fp} is
also popular.
%
While such approaches are ultimately inevitable,
formal verification is essential for
critical tasks such as 
aircraft collision avoidance verification~\cite{munoz-gappa-pvs}.
%
A higher degree of automation can greatly help with
these verification tasks.


An analysis method's ability to derive tight bounds is as important as
its ability to handle large expressions graphs.
%
Interval analysis provides an efficient and fast way to 
obtain error bounds; however, it inherently loses correlation
between terms, resulting in quite pessimistic bounds.
%
While affine analysis maintains correlations
between error variables by keeping them formal (symbolic), 
it can also result in  pessimistic bounds, especially for
non-linear expressions such as $x/(x+1)$, where the non-linearity
is introduced by division.


In this work, we introduce a scalable and rigorous approach
for error analysis embedded in a new tool, namely,
\satire({\bf S}calable
{\bf A}bstraction-guided {\bf T}echnique for {\bf I}ncremental {\bf R}igorous
analysis of round-off {\bf E}rrors). \satire supports scalable mixed-precision analysis and multi-output
estimation of straight-line
floating-point code.
%
We demonstrate that \satire can perform error estimation for
complex expression graphs involving thousands of operators, including
FFTs, recurrence equations, and partial differential equation (PDE) solving.



%while interval analysis~\cite{interval-anal}
%is very scalable, it can give quite pessimistic bounds
%(e.g., $(x-x)$ can return $[-2,2]$ when given $x\in [-1,1]$).
%%
%While affine analysis~\cite{affine-anal} maintains correlations
%between variables (and returns $0$ as the result of $(x-x)$),
%it also provides pessimistic bounds, especially for
%non-linear expressions such as $x/(x+1)$ where the non-linearity
%is introduced by division.


The recently proposed method of rigorously computing
{\em symbolic Taylor forms} and embodied in the
FPTaylor tool~\cite{DBLP:journals/toplas/SolovyevBBJRG19}
avoids problems associated with interval
and affine methods.
%
Moreover, as the table
of results in~\cite{DBLP:journals/toplas/SolovyevBBJRG19}
and \cite{DBLP:conf/sas/JacqueminPV18} show,
FPTaylor also produces some of the tightest bounds when compared
to the tools in its class.
%
However, FPTaylor cannot handle large expression graphs.
%
For example, for the discretized one-dimensional heat flow
(``1D-heat'') equation
calculation using a stencil whose temporal application
is unrolled over 10 time steps, about 442 expression nodes are
generated.
%
FPTaylor takes about 8 hours simply to generate the Taylor form expression,
following which its global optimizer fails to handle this expression.
%
In contrast, \satire handles the aforesaid 1D-heat problem
in a few seconds, generating tight bounds.
%
\satire also has handled expressions with over 200K operators
drawn from realistic examples.
%
In addition, \satire\ generates tighter error bounds than
FPTaylor on most of FPTaylor's examples.
%
To give an early indication of \satire's performance,
Table~\ref{tab:small-comparison} provides a sampling of examples
(comprehensive evaluations in \S\ref{sec:contributions}
and \S\ref{sec:eval}).

%% -- adding a small comparative table early on --
\begin{table}[htbp]
\centering
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Benchmarks} & \multirow{2}{*}{\# operators} & \multicolumn{2}{c}{Exec Time (secs)} & \multicolumn{2}{c}{Absolute Error} &
\raisebox{-4ex}{\shortstack[l]{Empirical Max\\ Abs Error}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & {\satire} & {FPTaylor} & {\satire} & {FPTaylor} \\
\midrule
jetEngine 			& 35 	& 1.969   & {\bf 0.84}	& {\bf 2.88E-08}	& 7.09E-08 & 1.57E-12\\
kepler2	  			& 43 	& {\bf 0.402}   & 0.52	&  3.20E-12		& {\bf 2.53E-12} & 3.49E-13\\
dqmom	  			& 35 	& {\bf 0.206}   & 0.63	& {\bf 9.66E-10} & 6.91E-05  & 3.27E-13 \\
1D-heat-10steps		& 442 	& {\bf 2.1} & - & 6.11E-15 & NA & 5.45E-16 \\
FFT-1024pt 			& 43K & {\bf 180} & - & 7.80E-13 & NA & 6.18E-15\\
Lorenz-20steps		& 307 	& {\bf 284} & - & 1.25E-14 & NA & 3.59E-15 \\
%fdtd1d-64steps		& 192k & {\bf 9711} & - & 7.45e-13 & NA & 9.89e-16\\
\end{tabular}
\label{tab:small-comparison}
\end{table}


%In this work, we provide a scalable
%and rigorous approach for error analysis embedded in a new tool
%\satire ({\bf S}calable
%{\bf A}bstraction-guided {\bf T}echnique for {\bf Incremental} {\bf R}igorous
%analysis of round-off {\bf E}rrors)
%that outperforms FPTaylor on virtually all of FPTaylor's benchmarks.
%
%
%--


The benchmarks Jetengine, Kepler, and DQMOM are some of the largest
that have been handled by FPTaylor, but contain no more than a few dozen
operators.
%
The much larger benchmarks including
FFT-1024pt (an FFT computation of 1K inputs),
and
Lorenz-20steps (a Lorenz system that captures the ``butterfly effect'')
%and fdtd1d-64steps (finite-difference time domain used in electromagnetic
%simulation and hundreds of other applications)
are all representative of practically important examples.
%
They far exceed the capability of all existing round-off error analysis
tools.
%
The last column of the table presents
the empirically calculated (using shadow values)
{\em maximum} absolute error over
$10^6$ simulations for randomly selected
data points from the input
intervals.
%
Lacking other means of easily obtaining tight rigorous bounds,
these results provide a good indication
of how close \satire's bounds
are.


\satire only analyzes for first-order error.
%
To check whether we are lacking precision due to this,
we ran FPTaylor on its own benchmarks with its second-order
error analysis turned off, only finding that the resulting error
values were still bit-identical.
%
This shows that it can be very difficult to
create examples where second-order error matters.
%
In~\cite{aiken-math-dot-h}, the authors further emphasize
this point by mentioning that they had to refine their
second-order error analysis beyond the approach taken in
FPTaylor.


\vspace{-1.6ex}
\paragraph{Roadmap:\/}
In \S\ref{sec:contributions}, we explain \satire's contributions
at a high level; this helps better understand the remainder of the paper.
%
In \S\ref{sec:contributions}, we explain the essential background
on floating-point arithmetic and the
global optimization-based error analysis done in \satire.%
%
We also point out the key contributions made by \satire.
%
In \S\ref{sec:illustrative-example}, we explain the
incremental analysis adopted in \satire.
%
\S\ref{sec:error-analysis} presents  the formal
details of \satire's error analysis with heuristics
for abstraction and for improving global optimization/canonicalization
detailed in \S\ref{sec:heuristics}.
%
\S\ref{sec:eval} presents a comprehensive evaluation of
\satire on many practical examples.
%
\S\ref{sec:relwork} presents additional related work.
%
\S\ref{sec:conc} has our concluding remarks.

%--end


==> old-text.tex <==
Here are some of the
highlights of \satire:
%
\begin{compactitem}
\item A 1024-point FFT with 43,083 nodes in its expression graph
      analyzed by \satire in 180 seconds obtaining a bound of {1.1e-12}
	  which is tighter than the previously known analytical bound of
	  {4.98e-12} ~\cite{fft-hal}.

\item The previously mentioned heat flow example was quite small.
      \satire tackled a 2D heat-flow example working on a 2D
      grid of 64 by 64 points
      iterated for 32 time steps to result in an expression
      graph of 270,402 nodes; \satire produced tight error
      bounds in under five hours.\footnote{The
      implementation of \satire is in Python, and is processed
      using a combination of standard Python (say which
      runtime), SimEngine (for expression canonicalization),
      and
      give more
      kingspeak details somewhere - a small summary here.
      Clearly, a custom C++ implementation and additional
               parallelization could be brought to bear
               to further reduce runtime.}

\item A one-dimensional
      finite-difference time-domain (FDTD) example---typically
      used for electromagnetic simulations---was unraveled for
      64 time-steps, resulting in an expression graph of
      192,811 nodes, with \satire solving it in under 2.7 hours.

\item We also measure the tightness of round-off errors estimated by
\satire (Section~\ref{sec:eval}) and show that it measures relative
error (and hence the number of mantissa bits ``lost'') fairly tightly.

%\item \skcmt{Include FFT precision result}
%
%
\end{compactitem}
%


\paragraph{\textbf{Floating point basics}}

A floating point number systems, $\mathbb{F}$, is a subset of real numbers representable
in finite precision and expressed as a 5 tuple $(\beta, s, m, e, p)$.
Here $\beta=2$ corresponds to the radix-2 floating point system with 
$p$ precision bits. Here $p=53$ and $24$ for double and single precision 
respectively, $s \in \{-1,1\}$ is the sign bit, $m$ is called the significand or
mantissa and $e$ is the exponent. There are two types of floating point
numbers, the {\em normals} and {\em denormals}, other than the special cases
of NANs and infinities. For the normal numbers $m$ lies in the range
$1 \leq m < 2$, while for the denormals the range is $0 \leq m < 1$.
%
The denormal range after the lowest {\em normal} number to make a gradual
transition towards zero. The exponent $e$ lies in a range $e_{\min} \leq e \leq e_{\max}$.
%
For double precision this range is $-1022 \leq e \leq 1023$.
%
Any such number, $\tilde{x} \in \mathbb{F}$ , has the value $s \cdot m \cdot \beta^e$.
%
If $x \in \mathbb{R}$, then $\tilde{x}$ denotes an element in $\mathbb{F}$
closest to $x$ obtained by applying the rounding operator($\circ$) to x.

IEEE754 defines four rounding modes for elementary floating point
operations. Every real number $x$ lying in the range of $\mathbb{F}$ can be
approximated by a member $\tilde{x} \in \mathbb{F}$ with a relative error
no larger than the unit {\em round-off} $\bf{u}=\dfrac{1}{2}\beta^{1-p}$.
%
Here, $\beta^{1-p}$ represents the {\em unit of least precision(ulp)} for 
the exponent value of 1. Thus, to relate the quantities $\tilde{x}$ and $x$
over the rounding operator, we have the following result
\begin{theorem}
	If $x \in \mathbb{R}$ lies in the range of $\mathbb{F}$, then
	\begin{equation}
	\label{eq:rounding}
	\tilde{x} = \circ(x) = x(1 + \delta),\quad |\delta| \leq \boldsymbol{u}
	\end{equation}
\end{theorem}

Note that based on the radix and precision, the round-off quantity varies.
We support mixed precision analysis, hence we will suffix the rounding
operator when necessary to denote the precision for the rounding. For example, when rounding
in double precision we denote $\circ_{32}$.
%

Given two exactly represented floating point numbers, $\tilde{x}$ and $\tilde{y}$,
arithmetic operators $\diamond in \{+,-,\times,/\}$ have the following guarantees
\begin{equation}
\label{eq:opbound}
\begin{split}
	\circ(\tilde{x} \diamond \tilde{y}) &= (\tilde{x} \diamond \tilde{y})(1 + \delta),\quad |\delta| \leq \boldsymbol{u} \\
	&= (\tilde{x} \diamond \tilde{y}) + (\tilde{x} \diamond \tilde{y})\delta \\
	&= \{ \hbox{real value} \} + \{ \hbox{ round-off error } \}
\end{split}
\end{equation}

Thus the rounded result involves an interval centered around the real exact value where the
width of this interval is determined by the amount of round-off error accumulated.

Besides the elementary operators, \satire supports other complex mathematical
operations like transcendentals. In such cases, the bound on the $\delta$ terms changes
as a multiple of $\bf{u}$. We keep a default value for each operator, but it is
configurable, hence allowing the user to obtain customized error bounds
for the specific math library being used.

\paragraph{\textbf{Affine Analysis}}
In an affine arithmetic, a quantity $\hat{x}$ is represented in an affine form as 
$\hat{x} = x_0 + \sum_{i=1}^n x_i \epsilon_i$, where $x_0$ denotes the central value
and the $x_i$'s are finite floating point numbers representing noise coefficients
associated with the corresponding noise variables, $\epsilon_i$'s. The $\epsilon_i$ are
formal variables whose value lies in [-1,1] but unknown until assigned. This representation
allows for cancellations occuring on converging paths to cancel out error terms thus improving
tightness. For example $(x-x)$ in AA will yield 0 because the noise variables can cancel
each other unlike in interval analysis where they keep widening the intervals.

In \satire, we apply affine analysis in a modified way.
Instead of $x_i$ components being
evaluated finite floating point numbers, we preserve them as symbolic terms.
Symbolic taylor forms comprise of two parts generated in one shot, that is the composition of the error term and the derivatives. \satire {\em decouples} this method into separate passes. A forward pass for generating symbolic error terms at each operator site and a backward pass of obtain symbolic derivatives. The decoupling logic is key to \satire's efficiency since it does not requires to carry forward all error variable to the output node unlike FPTaylor.
Besides saving the computational cost of the noise coefficients at every node,
it enables our simplification procedures for canonicalization of expressions. 
%
Since at every node, the error(noise) coefficients
are symbolic, similar variable terms can be grouped
together for simplification(canonicalization). 
Interval based global optimizers(such as ours and FPTaylor's)
show better convergence when occurence of the same variable in isolation
is reduced, that is, $x^2$ converges better than $x*x$.
Hence, \satire stresses heavily on effective canonicalization
of expression that are fed to the optimizers.




%while interval analysis~\cite{interval-anal}
%is very scalable, it can give quite pessimistic bounds
%(e.g., $(x-x)$ can return $[-2,2]$ when given $x\in [-1,1]$).
%%
%While affine analysis~\cite{affine-anal} maintains correlations
%between variables (and returns $0$ as the result of $(x-x)$),
%it also provides pessimistic bounds, especially for
%non-linear expressions such as $x/(x+1)$ where the non-linearity
%is introduced by division.
%In this work, we provide a scalable
%and rigorous approach for error analysis embedded in a new tool
%\satire ({\bf S}calable
%{\bf A}bstraction-guided {\bf T}echnique for {\bf Incremental} {\bf R}igorous
%analysis of round-off {\bf E}rrors)
%that outperforms FPTaylor on virtually all of FPTaylor's benchmarks.



===


\skcmt{Complex sentence}
\satire implements a hybrid usage of techniques over
interval and affine analysis. It symbolically propagates
function and error expressions
over input variables to allow preserving correlations of
variables and error terms in the forward path. Additionally,
it allows to abstract internal nodes at selected points inside the AST
by obtaining numerical error bounds for those nodes such that these
nodes can be used as free variables(leaf nodes) in the forward path.
One one hand, if every node in the AST had been abstracted, this would be equivalent
to a worst case interval analysis with heavily bloated
error bounds. On the other hand, if we solved for the interval of each
symbolic error term generated at every operator site followed by their propagated and
accumulation at the output node, it will be equivalent to a complete affine analysis.
%input variables combined with generation 
%and propagation of errors over symbolic expressions.
%Tools like gappa~\cite{munoz-gappa} use interval analysis with theorem
%provers while rosa~\cite{rosa} and fluctuat~\cite{fluctuat}
%employ affine analysis.

We provide background on floating-point arithmetic and affine analysis
 followed by an intuitive overview of our approach.

%
%-- \input{floating-background.tex}



 ===

 
\adcmt{The preceding or the next sentence?}
The denormal range begins after the lowest {\em normal} number to make a gradual
transition towards zero. The exponent $e$ lies in a range $e_{\min} \leq e \leq e_{\max}$.
%
===



\begin{comment}
A radix-2 floating point {\em normal} number (numbers whose
mantissae are of the form ``$1.m$'')
for a precision
$p$ (typically $p=32$, called single precision,
or $p=64$, called double precision) helps define a proper subset of
real numbers via a sign bit $s$, a mantissa word $m$ (23 bits
for single 52 for double) and an exponent word $e$ (8 bits for single
and 11 for double) via the formula $(-1)^s\cdot (1.m) \cdot 2^{e}$.
%
Subnormal numbers
are of the form $0.m$
and represent values below $2^{-126}$ (single) and below $2^{-1022}$ (double).
%
When rounding error is treated as ``noise''
and one performs a Taylor expansion, one is often concerned with
the {\em first-order error} which is what \satire estimates.
%
Second order error as well as subnormal values are of the same order,
are quite small, rarely matter,
and hence ignored in this work.\footnote{See
Section~\ref{sec:relwork} for discussions on where they don't matter
and where they do.}



IEEE754~\cite{ieee754} defines four 
rounding modes, of which we primarily consider {\em round to nearest}.
%
Define $\epsilon$ to be the {\em unit round-off} (the constant
$2^{-24}$ for single and $2^{-53}$ for double).
%
As per the first-order round-off error model, a calculation
such as $(x+y)$ introduces an error $(x+y) \epsilon$.\footnote
{We can be very specific about each operator's unit-roundoff: thus,
 $\epsilon_{+}$ would be more accurate.}
%
There is another concept called {\em unit in the last place} or $ulp$
whose magnitude is the least resolution at a particular value; in
particular, $ulp(1)=2\epsilon$, and doubles every binade (whenever the
exponent increases by 1). \skcmt{ulp definition is unclear. Can we use a more intuitive definition?}


In general, rounding errors are most serious when values
with very high exponent differences
are combined (e.g., added).
%
Often, a value with a very low exponent magnitude can disappear entirely.
%
Given that half of the representable floating-point numbers exist
in the interval $[-1,1]$,
there are many binades present in the interval $[0,1]$ and hence
for benchmarking examples, this forms a meaningful interval of inputs
to apply (and used in many of our examples).
%
If one wants to study benchmarks without much binade spread,
one can choose intervals such as $[1,2]$ within which
the values are apart by at most one binade. \skcmt{Is this what we do? If not, this is an odd proposition to put forth.}



\skcmt{Higher precision does not imply exact solution; so we could say ``get close to'' rather than obtain}
%
Given a floating-point expression,
one can obtain its ``true value'' (close to its real number value)
either by employing higher precision shadow value calculations
or libraries such as MPFR~\cite{mpfr}. 
%
The ``computed value'' is the one obtained after rounding
in the working precision.
%
{\em Absolute error} refers to the absolute difference between the
true and computed values, while
{\em relative error} is absolute error divided by the magnitude
of the true value.
%
Relative error provides a direct indication of the number of bits
lost due to rounding.\footnote{Unless the
true answer is close to $0$.}
%
In particular, for relative error $r$, the number of bits lost due
to rounding, $lost(r)$, equals $log_2(r/ulp(1))$.
%
This result captures the number of mantissa bits
necessary to represent the relative error
in terms of the number of $ulp(1)$ steps.


Given all this, it is possible to employ
\satire to estimate the maximum number of mantissa bits
lost (in support of precision profiling) as follows.
%
The answer produced by \satire is the estimated
absolute error.
%
Therefore,
if we manage to observe a value $v$ during an actual computation
and the \satire-estimated absolute error is $e$,
then one can take $v$ to be ``true value''
(as it happens to be observed in the real system)
and estimate the number of bits lost as $lost(e/v)$.
%
\skcmt{I don't get this argument. Above we say true value is exact, here we say true value is what us observed.}
%
We use these ideas in our results presented in
Section~\ref{sec:eval}.
\end{comment}

\begin{comment}
We now provide some insight into how
the symbolic Taylor Form approach works.
%
Consider the expression $(E_1+(E_1+E_2)$ where
$E_1$ and $E_2$ are complex 
%
The Symbolic Taylor Form approach
introduces ``noise'' variables at each operator
to model rounding.
%
%
In particular, the error-laden counterpart of 
$E_0 = x+(x+y)$ is modeled as
$E=(x+(x+y)(1+\epsilon_1))(1+\epsilon_2)$, where the magnitude of
$\epsilon_1$ and $\epsilon_2$ are bounded by $\epsilon$.
%
One can expand this expression using Taylor expansion
to reveal the first order error terms:
\( E = E_0
       + \epsilon_1 \cdot \frac{\partial E}{\partial \epsilon_1}
       + \epsilon_2 \cdot \frac{\partial E}{\partial \epsilon_2}
\)
%
Notice that $(E-E_0)$ is the absolute error.
%
Tools such as FPTaylor, Real2float, and Precisa rely on
{\em global optimizers} to compute the supremum of the
absolute error expression $(E-E_0)$.
%
%
Gelpia~\cite{fptaylor-toplas},
the global optimizer used in FPTaylor,
is based on
{\em interval branch and bound} (IBB~\cite{french-paper})
and relies on an efficient interval-arithmetic
solver~\cite{gaol} to estimate the bounds.


IBB tools rely on the key property of {\em interval
  monotonicity}:
for every operator $f$ used in the expression being
optimized, and for
intervals of real values $A$ and $B$ where
$A\subseteq B$, we must have $f(A)\subseteq f(B)$.
%
This monotonicity property
allows IBB-based tools to subdivide their input domains
and search over the population of subdivided domains.
%
Usually a heuristic (a genetic algorithm) guides the search,
and must be tuned with additional heuristics to properly
converge.
%
It is worth emphasizing that if this global optimization
process is not properly handled, two things can go wrong:
(1)~tight error bounds may not be obtained,
and
(2)~the optimization time can be enormous.
%
These are the points that \satire emphasizes.


It is worth observing from
$(E-E_0)$
that 

error anaysis on $E_1+(E_1+E_2)$,
one can either analyze this expression as such, or converted it
to $(E_1+E_1)+E_2$ and analyze---or even
convert it to $2E_1+E_2$ and analyze.
%
Are these choices equivalent?
%
Given that floating-point arithmetic does not obey
standard algebraic rules such as associativity,
the answer is ``no'' in general.
%
Floating-point arithmetic is also non-compositional.
%
For example, one can find input intervals for $x$
for which $(e^x-1)/x$ has {\em worse}
error than
$(e^x-1)/log_e(e^x)$~\cite{kahan}!


{\em More than the lack of associativity and lack of compositionality}, 
one must also keep in mind the ``quirky'' behavior of global
optimizers.
%
This problem is well-recognized in the global optimization
literature~\cite{cite-paper-benchmarking-global-opt}.
%
More specifically, for IBB-based global optimizers,
the answer is returned after a bounded number of steps
of search.
%
In this context,
it is important to keep
in mind that for examples with many suprema, it is important to
{\em canonicalize expressions before submitting to a global
optimizer}.
%
For example, if we submit $x*x$ for $x\in[-1,1]$ to Gelpia,
we find that it gives the answer $[-1,1]$ while if we feed
$x^2$, it returns $[0,1]$.
%
It is quite likely that $2E_1+E_2$ will return a far better
bound than
$E_1+(E_1+E_2)$  or
$(E_1+E_1)+E_2$.
%
In a nutshell,
  {\em \satire's tightness of bounds is critically dependent
  on these canonicalizations.}
%
Except for some rare corner cases of functions with many
local maxima/minima, canonicalizations almost always help,
and {\em is the key step to \satire's success with providing
  tight bounds, despite its scalability}.


(THIS CAN BE MOVED TO ANOTHER PLACE...)
\begin{sf}
  These correlations are so important in \satire that
we now highlight another situation where it is exploited.
%
When we add up the path contributions of errors at each backward
%
derivative application, we can either
do sum(abs(exps)) or abs(sum(exps)), and the latter is far better
as it canocalizes the term {\tt sum(exps)} to a significant extent.
%
If we were to do {\tt sum(abs(exps))}, we keep the exps apart
via the {\tt abs} function; they are ``insulated'' from each
other, resisting being combined.
%
Thus, while
sum(abs(exps)) and abs(sum(exps)) are real-equivalent, they
are not ``global optimizer equivalent.''
\end{sf}

 %--
\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{figs/introEx.pdf}
  \end{center}
  \caption{An Example Expression DAG}
  \label{fig:introEx-dag}
\end{wrapfigure}
%--


(ALSO TALK ABOUT reverse mode AD ideas with the help of the figure...)

The approach used in \satire is illustrated with the help of the
expression in Figure~\ref{fig:introEx-dag}.
%

Describe how the local error is generated at (y-x) and propagated
up the shown path via the reverse-mode AD.

Say we do an abstraction at *, we have x uncorrelated.

Stop with a solid connection between what we do in reverse-mode AD
and what FPTaylor does.


\end{comment}


==
\ggcmtside{If you want more exact numbers, in 17 examples FPTaylor got better results
while in 28, Satire got better results.
I also put the ``*'' for one or more order of magnitude of separation.
We can obtain a weighted summary if we include
say AST nodes. Or maybe talk about the number of orders of magnitude better ... or something.
Maybe best to leave such weighted summaries but
maybe include other classifications---e.g. for type ``X'' of examples,
Satire is always far better.}

%
%Complex numbers introduces difficulties for
%traditional error analysis tools to handle such expressions.
%
%, requiring specialized backend 
%optimizer supporting complex numbers. At this point we are not aware
%of any such tools that supports error analysis for complex expressions.

As noted earlier, linear systems  such as FDTD
can be simplified over larger operational counts (as large as 30k) and 
optionaly available as a knob to the user.


==> scan.tex <==
\paragraph{Prefix Sum: } Prefix sum or simply scan of a sequence of numbers that generates
another sequence by finding the sum of prefixes or running totals of the original sequence.
If $x_1, x_2,\dots, x_n$ is the input sequence and $y_1, y_2, \dots, y_n$ is the output 
sequence, then prefix sums generate the sequence as $y_i = y_{i-1} + x_i$ with $y_1 = x_1$.
It takes advantage of the assosiativity of the `sum' operator to parallelize the prefix sum evaluations with wide randing applications in stream compaction and sorting algorithms ~\cite{prefixsum}. 

The prefix sum benchmark performs a scan operation on an input sequence of 1024 data points.
This scan algorithm performs an initial upsweep followed by a downsweep to compute the
entire output sequence. We estimate the error on the output point having the largest datapath.
Since floating point compute is non-compositional, error analysis on summation algorithms
needs to take care of the ordering of the operations, otherwise a generic bound as ~\cite{boldo} will be too conservative to be of any use. \satire reports an error bound of 1.88e-12
for all the data points in the $[0,1]$ range while being little shy of 3 minutes in execution 
time while FPTyalor times out while building the taylor forms. Furthermore, we obtain
the same bound with abstraction enabled within 30 seconds showing the effectiveness
of our abstraction techniques.



==> sriram-intro.tex <==
Numerical software systems modeling scientific and engineering applications
rely heavily on finite-precision arithmetic while being designed for
real arithmetic algorithms.
%
As a result, when computed in finite precision, the computations
accumulate approximations due to
rounding errors.
%
Hence, rigorous analysis of these round-off errors becomes important
to ensure the programs are operational within known 
error bounds, preventing events  such as
inaccuracies in statistical computing and econometric software
leading to market crashes~\cite{economic, numstats} or the more
catastrophic patriot missile failure~\cite{patriot-missile}, 
%explosion of the Ariane rocket ~\cite{bad-numerics-examples}, 
all stemming from unaccounted floating-point inaccuracies.

Those interested in {\em verification}
typically focus on rigorously bounding the round-off error to be within 
chosen limits (an important step in verifying
 many hardware/software systems
 % ~\cite{darulova-cps}
 ~\cite{rosa}
 and cyberphysical systems
 %~\cite{titolo-munoz-winding-number}).
 ~\cite{munoz-winding}).
%
Those focused on {\em tuning} typically combine
 different implementations (e.g., single
 and double precision computations)
 of floating-point functions to achieve
 an overall implementation that achieves given round-off error targets
 while reducing the overall computational cost
 (important for improving
  energy consumption and performance
  %~\cite{some-other-rigorous-tuning,fptuner,precimonious}).
  ~\cite{adapt,fptuner,sc13-precimonious}).

%Floating-point arithmetic is widely employed across many scientific
%and engineering applications.
%%
%Rigorous analysis of the round-off error introduced by floating-point
%operations is important in many contexts.
%%
%Those interested in {\em verification}
%typically focus on rigorously bounding the round-off error to be within 
%chosen limits (an important step in verifying
% many hardware/software systems~\cite{darulova-cps}
% and cyberphysical systems~\cite{titolo-munoz-winding-number}).
%%
%Those focused on {\em tuning} typically combine
% different implementations (e.g., single
% and double precision computations)
% of floating-point functions to achieve
% an overall implementation that achieves given round-off error targets
% while reducing the overall computational cost
% (important for improving
%  energy consumption and performance~\cite{some-other-rigorous-tuning,fptuner,precimonious}).
%%
%Another application is
% {\em precision profiling} in which
% one tries to estimate the relevant number of 
% mantissa bits as a computation proceeds.
%%
%Precision profiling methods
%(e.g., \cite{verificarlo,verrou}) allow one to understand
%opportunities for changing the working precision.



Unfortunately, even the best of today's {\em rigorous} and
{\em automated} round-off error
estimation tools can only handle expressions with a few hundred
operators
%~\cite{toplas-paper-tool-citations,fpbench-examples}.
~\cite{fptaylor,fpbench}.
%
They cannot handle
larger expressions involving thousands of operators
that arise in many practical designs
such as schemes to solve recurrence equations~\cite{lorentz},
important algorithms such as the Fast
Fourier Transform (FFT), parallel prefix sum (scan) algorithms
or stencil computations involving iterative solvers and partial 
difference equations(PDEs).
%
Current approaches for {\em scalable} rigorous
analysis employ a combination of abstract interpretation and
theorem-proving
methods
%~\cite{fluctuat,winding-number,more-refs,munoz-gappa-pvs,boldo-2nd-order-wave}
~\cite{fluctuat,munoz-winding,munoz-gappa,boldo-2nd-order-wave},
all of which involve manual effort.
%
Given the lack of rigorous and {\em automated}
tools that
scale, many settle for sampling-based
methods~\cite{sc13-precimonious,hifptuner,herbie,craft}
to estimate errors on chosen input points or %and tune the implementation,
estimate working precision based on Monte Carlo
sampling~\cite{verificarlo}.%, etc.
%
These methods come with no formal guarantees on the unexamined
inputs.

%% Introduce Satire here ... then in following text build contardictions with 
%% Satire for every new pointers of discussion

In this work, we introduce a scalable and rigorous approach
for error analysis embedded in a new tool
\satire({\bf S}calable
{\bf A}bstraction-guided {\bf T}echnique for {\bf I}ncremental {\bf R}igorous
analysis of round-off {\bf E}rrors). \satire supports scalable mixed-precision analysis and multi-output
estimation of straight-line
floating-point code.
%
We demonstrate that \satire can perform error estimation for
complex expression graphs involving thousands of operators, including
FFTs, recurrence equations, and PDEs.

An analysis method's ability to derive tight bounds is as important as
its ability to handle large expressions graphs.
%
Error analysis methods that are rigorous but only provide fairly
loose error bounds are useless in practice.
%
Interval analysis provides an efficient and fast way to 
obtain error bounds but inherently loses correlation
between terms resulting in quite pessimistic bounds.
On the other hand, affine analysis maintains the correlations
between error variables by keeping them formal (symbolic). 
However, this can also result in  pessimistic bounds, especially for
non-linear expressions such as $x/(x+1)$, where the non-linearity
is introduced by division.
%while interval analysis~\cite{interval-anal}
%is very scalable, it can give quite pessimistic bounds
%(e.g., $(x-x)$ can return $[-2,2]$ when given $x\in [-1,1]$).
%%
%While affine analysis~\cite{affine-anal} maintains correlations
%between variables (and returns $0$ as the result of $(x-x)$),
%it also provides pessimistic bounds, especially for
%non-linear expressions such as $x/(x+1)$ where the non-linearity
%is introduced by division.
%
The recently proposed method of rigorously computing
{\em symbolic Taylor forms} and embodied in the
FPTaylor tool~\cite{toplas}
avoids both problems. % associated with interval
%and affine methods.
%
Moreover, as reported in ~\cite{FPTaylor-toplas,DBLP:conf/sas/JacqueminPV18},
FPTaylor also produces some of the tightest bounds across
a spectrum of benchmarks
when compared against the following tools:
Fluctuat~\cite{fluctuat}, Gappa~\cite{gappa},
PRECiSA~\cite{precisa}, Real2Float~\cite{real2float},
Rosa~\cite{rosa}, and
Numerors~\cite{DBLP:conf/sas/JacqueminPV18}.


However FPTaylor does not scale to handle
expression graphs that arise even in small benchmarks.
%
For example, for the discretized one-dimensional heat flow
(``1D-heat'') equation
calculation using a stencil whose temporal application
is unrolled over 10 time steps, about 442 expression nodes are
generated.
%
FPTaylor takes about 8 hours simply to generate the Taylor form.
Subsequently,
the global optimizer that comes with FPTaylor gives up on
this Taylor form.


%In this work, we provide a scalable
%and rigorous approach for error analysis embedded in a new tool
%\satire ({\bf S}calable
%{\bf A}bstraction-guided {\bf T}echnique for {\bf Incremental} {\bf R}igorous
%analysis of round-off {\bf E}rrors)
%that outperforms FPTaylor on virtually all of FPTaylor's benchmarks.
%
%
%--
\begin{figure}
	\centering
    \includegraphics[width=1.0\textwidth]{figs/gradual-abstraction-illustration.PNG}
  \caption{Incremental error analysis using gradual abstraction}
  \label{fig:gradual-abstraction}
\end{figure}
%--
%

\satire scales far better than all tools we are aware of.
%
For example, \satire handles the aforesaid 1D-heat problem
{\em in a few seconds.}
%

\satire improves scalability by introducing a notion of
{\em node abstraction} that incrementally guides the  
forward error analysis.%
Figure~\ref{fig:gradual-abstraction} illustrates the incremental abstraction scheme
using
%the node abstraction.
%
%It shows
an iterative stencil's evolution in time.
%
Two successive abstractions are performed, followed by a direct computation of the
final output error.
%
Intuitively, \satire builds symbolic error expressions
feeding into a global optimizer for obtaining the maximum error.
%
\skcmt{The following sentences are very difficult to follow.}
%
These symbolic error forms begins to get large and complex with increasing AST depth,
number of input variables and for non-linear expression types, which further bottlenecks
the backend optimizer.



%obtain
%increases
%To counter the explosion of the symbolic expressions for large AST
%depths and interconnected networks, 
%it partitions the AST using a cost-metric
%guided heuristic and employs user knobs to abstract the compute nodes
%at designated `cut' points. These selected nodes are solved in isolation
%for their errors and the AST is rebuilt with these nodes as free variables
%with an in-flowing error term.
Our results
in Section~\ref{sec:eval} show that \satire can handle a variety
of problems
of very large expression sizes, while producing tight guarantees.

Table~\ref{tab:small-comparison} highlights the performance 
of \satire as compared to FPTaylor for selected benchmarks (additional benchmarks are presented in Section~\ref{sec:eval}). 
jetengine, kepler, and dqmom are benchmarks from FPTaylor's suite with relatively
large operator counts. heat, fft, lorentz (non-linear), and fdtd are added
to show \satire{}'s performance for even larger operator
counts. % enabling insights into more complex systems forming building blocks
%of numerical kernels in scientific computing applications.
%
FPTaylor is unable to handle such large expressions
%more common in HPC systems. 
common in many practical situations.

%% -- adding a small comparative table early on --
\begin{table}[htbp]
\centering
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Benchmarks} & \multirow{2}{*}{\#operators} & \multicolumn{2}{c}{Exec Time(seconds)} & \multicolumn{2}{c}{Absolute Error} & Empirical Max\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & {\satire} & {FPTaylor} & {\satire} & {FPTaylor} & {Abs. Error}\\
\midrule
jetEngine 			& 35 	& 1.969   & {\bf 0.84}	& {\bf 2.88E-08}	& 7.09E-08 & 1.57e-12\\
%kepler2	  			& 43 	& {\bf 0.402}   & 0.52	&  3.20E-12		& {\bf 2.53E-12} & 3.49e-13\\
%dqmom	  			& 35 	& {\bf 0.206}   & 0.63	& {\bf 9.66E-10}* & 6.909e-05  & 3.27e-13 \\
%heat1d-10steps		& 442 	& {\bf 2.1} & - & 6.1062e-15 & NA & 5.45e-16 \\
kepler2	  			& 43 	& {\bf 0.40}   & 0.52	&  3.20E-12		& {\bf 2.53E-12} & 3.49e-13\\
dqmom	  			& 35 	& {\bf 0.21}   & 0.63	& {\bf 9.66E-10}* & 6.90e-05  & 3.27e-13 \\
heat1d-10steps		& 442 	& {\bf 2.1} & - & 6.10e-15 & NA & 5.45e-16 \\
FFT-1024pt 			& 43k 	& {\bf 180} & - & 7.80e-13 & NA & 6.18e-15\\
Lorentz-20steps		& 307 	& {\bf 284} & - & 1.25e-14 & NA & 3.59e-15 \\
fdtd1d-64steps		& 192k & {\bf 9711} & - & 7.45e-13 & NA & 9.89e-16\\
\bottomrule
\end{tabular}
\caption{\satire is more scalable than FPTaylor with, often, improved error bounds. Boldface denotes the better scheme for each benchmark. \label{tab:small-comparison}}
\end{table}
%%

The last column of Table~\ref{tbl:small-comparison} shows the empirically seen
maximum absolute error over
10,000 simulations of each kernel for randomly
distributed data points in the specified interval. For the kernels where
a comparable bound from FPTaylor is unavailable, the emprirical bound
statistically shows the tightness of \satire's bounds.
Consider the case for `dqmom', where \satire's bounds are much tighter
than the previously reported FPTaylor bounds. 
Multiple occurences of the same variable loses correlation
when treated with interval-based optimizers.
%
\skcmt{Above it is said FPTaylor is not affected by this problem affecting interval analysis. So the preceding statement is conflicting/confusing.}
\adcmt{I think it appeared to be confusing. Earlier it is said FPTaylor produces tight results compared to the other mentioned tools. The simplification issue for interval based solver for the optimizer still exists, that being a separate issue that using interval analysis for error propagation. I agree this part needs to be clarified upfront.}
%
\satire stresses the use of {\em simplifying
symbolic expressions} to reduce the individual occurrence of a variable
term. Here each symbolic expression is comprised 
of unique symbols representing an input variables or an abstracted node(as a free variable) such that each variable has an associated incoming error term and a numeric interval.  
%
\skcmt{do you mean repeated occurrence of a variable?
Also ``variable term'' is not defined thus far.}
%
We refer to this process as {\em canonicalization} or {\em
simplification}.
%
\skcmt{Given an idea of canonicalization.
Not good to leave it as a magic sauce.
Following sentence in unclear. Not sure how to improve it.}
\adcmt{Will add this in final intro, or Professor is going to add this
as part of his reorg we discussed earlier}
%
Feeding the optimizer with the synthesized expressions optimized for
preserving correlation (through canonicalization) aids better
convergence results for \satire.
%
\adcmt{Remove highlights as points ... discuss the table}
\adcmt{Change unique features to format as contributions}
Here are some of the
highlights of \satire:
%
\begin{compactitem}
\item A 1024-point FFT with 43,083 nodes in its expression graph
      analyzed by \satire in 180 seconds obtaining a bound of {1.1e-12},
	  a tighter than the previously known analytical bound of
	  {4.98e-12} ~\cite{fft-hal}.

\item The previously mentioned heat-flow example was quite small.
      \satire tackled a 2D heat-flow example working on a 2D
      grid of 64 by 64 points
      iterated for 32 time steps, an expression
      graph of 270,402 nodes; \satire produced tight error
      bounds in under five hours.\footnote{The
      implementation of \satire is in Python, and is processed
      using a combination of standard Python (say which
      runtime), SimEngine (for expression canonicalization),
      and
      give more
      kingspeak details somewhere - a small summary here.
      Clearly, a custom C++ implementation and additional
               parallelization could be brought to bear
               to further reduce runtime.}

\item A one-dimensional
      finite-difference time-domain (FDTD) example---typically
      used for electromagnetic simulations---was unraveled for
      64 time-steps, resulting in an expression graph of
      192,811 nodes, with \satire solving it in under 2.7 hours.

\item We also measure the tightness of round-off errors estimated by
\satire (Section~\ref{sec:eval}) and show that it measures relative
error (and hence the number of mantissa bits ``lost'') fairly tightly when
compared with a high precision shadow value calculation.
\skcmt{If this is empirical comparison, would be good to state that here.
Otherwise, the reviewers might expect ground truth comparison.}

%\item \skcmt{Include FFT precision result}
%
%
\end{compactitem}
%
Thus, \satire can
serve as a stand-alone error-bound verifier for large expressions,
or be used as a primitive tool within a theorem-proving context
(when it may help reduce the number of proof-decomposition
      steps).
%      
It can also help in the roles of
rigorous precision profiling
and provide precision tuning.


\subsubsection{Unique Features of \satire}

\satire's design takes advantage of the best of many
existing approaches, while adding its own set of unique directions:

%--
\begin{compactitem}
\item It combines interval analysis and symbolic analysis to
      achieve a good
      tradeoff between scalability and correlation of errors.

\item \satire performs
      {\em canonicalization} of expressions during symbolic
      analysis that allows
      its back-end global-optimizer to converge to
      tight error bounds.
      %
      The effectiveness of canonicalization was confirmed
      by applying this step to the Symbolic Taylor Forms
      produced by FPTaylor whereupon
      the error bounds became tighter
      (we discuss this in Section~\ref{sec:eval}).
      
\item It supports the ability to
      create abstractions of large
      subexpressions
      during forward symbolic evaluation
      (explained in Section~\ref{sec:absguided})
      based on user-specified cost metrics.
      %
      Section~\ref{sec:eval} shows that the error estimates
      following abstraction
      are still quite informative (not grossly exaggerated)
      in most cases.

\item Most important of all,
      \satire   performs error calculations
      {\em incrementally}
      while walking the expression
      graph---instead of the monolithic approach taken in
      tools such as FPTaylor.
      %
      This is a major reason why \satire achieves scalability.
\end{compactitem}

\noindent{\bf Roadmap:\/}

ROADMAP of the paper

\begin{comment}

% intro

Any formal activity involving floating-point expressions---be it formal
verification, rigorous precision tuning, or some other---centrally relies
on our ability to provide {\em tight} error bounds for {\em large}
expressions.
%
Unfortunately, even the best of today's methods suffer from the following
drawbacks: (1)~they can provide tight bounds, but for small expressions
using methods such as affine analysis combined with symbolic (SMT)
reasoning~\cite{eva,others,dont-forget-thomas-wahl},
Taylor forms~\cite{taylor-forms},
or other methods~\cite{other-methods};
(2)~they can provide loose bounds for larger expressions, either using
interval-based methods~\cite{some-intvl-methods}, empirical (sampling)
methods~\cite{all-sampling-based-prec-analysis-such-as-in-sc19-tut}, or
statistical methods such as Monte-carlo arithmetic~\cite{mca}.
%
There are {\em no available} methods that handle multi-output expressions
involving, for instance, 4,000 inputs and 
involve expression DAGs with a maximum depth of hundreds.
%
These are the kinds of expressions one can obtain in many practical
situations.
%
Some of the situations that give rise to such expressions include:
%
\begin{compactitem}
\item Unraveled arithmetic computations such as
  parallel prefix sums (scan), stencil-based computations for
  solving partial differential equations (PDE) or optimized implementations
  algorithms of central importance such as FFT.

\item Recurrences that model the solutions of equations based on Newton's
  method~\cite{newton} or
  standard benchmarks with highly unstable trajectories such
  as Lorenz attractors~\cite{lorenz}.
\end{compactitem}
%
Unfortunately, today's precision analysis methods simply cannot deal
with these sort of expressions unless they heavily employ (unsound)
underapproximations that often rely on shadow-value calculations
on a limited number of input points, or highly useless bounds obtained through
interval branch-and-bound search algorithms.
%
This prevents recent advances in floating-point reasoning and tuning from
handling sizes that practitioners would care.


  In this paper, we provide a novel hybrid approach that synergistically combines
  multiple ideas to achieve this goal.
  %
  In particular, our work combines the best features of
  many methods including symbolic execution,
  automatic differentiation,
  interval analysis, 
  and guided abstraction.
  %
  Our method implemented in a new tool Satern can handle very large expressions
  with BIGNUM expression DAG nodes.
  %--
  Such results are being obtained in the area of formal analysis of floating-point
  arithmetic for the first time.


  (Say more.)
  
\end{comment}






==> stencil.tex <==
\paragraph{Stencils: } Stencils belong to an important class of 
iterative solvers operating on dense arrays modeling partial
difference equations with applications ranging from 
fluid dynamics, cosmology, combustion, etc. 
%
They form essential building blocks for solving
larger more composite problems and as such knowledge 
of the accumulated round-of errors are of importance 
for ensuring overall correctness.
%
However, these comprise of
large and dense arrays being updated over time and
involving spatial dependencies between the grid points
as shown in figure ~\ref{fig:iteratedStencil} for a 3-point stencil.
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figs/iteratedStencil.png}
  \end{center}
  \caption{Iterative structure of a 3 point stencil}
  \label{fig:iteratedStencil}
\end{wrapfigure}

There are 2 key features presents in such computational update schemes
which makes obtaining a tight and rigorous error bound critical. 
%
Firstly, each point in this system contributes to a set of
neighbouring points in the immediate future
as per the arity of the stencil.
%
Thus, an error term(round-off or otherwise)
generated locally at a certain grid point will effectively 
spread across the compute space as the simulation progresses.
%
Secondly, there are many interconnected contributing terms emanating from 
a point that merge in the forward path. It implies preserving correlations
when forming error expression is essential for such computations.
%
This is because pure interval analysis will move the needle towards 
widening error intervals due to the spatial spread of
contributions. However, preserving correlations symbolically or
using affine analysis will bring back correlations for tighter bounds.
Even so, obtaining a quantifiable error bound in such applications becomes 
important atleast over few iterations of the application which allows the 
developers a level of confidence in its numerics.
%

Absence of tools to provide rigorous bounds for such applications forces developers to
resort to empirically validating the numerics using shadow value computations
or rely on statistically obtained precision qualities, neither of which are 
provavbly rigorous.
%
When applied to existing tools , they are faced with the difficuly in handling
such interconnected computational structures even for few iterations. For example,
solving for a one dimensional heat stencil formed by unrolling the stencil structure of figure ~\ref{fig:iteratedStencil}  for only 
10 iterations requires FPTaylor executing for almost 8 hours to complete its
symbolic taylor form building stage. Inherently this means we cannot apply
such rigorous tools for any practical cases of these examples required to
iterate over atleast 100 of iterations and even more-so for multidimenisonal cases 
of these problems.
%

\satire can solve the above stencil benchmark comprising of around 400 operations
within 4 seconds obtaining an absolute error bound of 6.10e-15. Unrolling this
stencil for 32 iterations results in 4226 compute nodes and requires a solving
time of 170 seconds with an absolute error bound o 1.95e-14. We further unroll the stencil
to 128 iterations involving 66050 operations. The backend optimizer encounters
difficulty in processing such a large query, hence we enable our abstraction techniques leading to a solution of 7.8e-14 while taking arounds 40 minutes to solve. Note that while 
abstraction guided tecniques helps us to tackle large problems, it may
significantly increase the number of optimization queries necessary to absract the internal 
nodes, specifically in cases like stencils where there are a large number of nodes to be abstracted at a given depth.

%% add a result without partial solve



==> unclear-writing.tex <==


Consider for instance the DQMOM example where \satire's bounds are
tighter by five orders of magnitude compared to previously reported FPTaylor bounds.

Multiple occurences of the same variable loses correlation
when treated with interval-based optimizers.
%
\skcmt{Above it is said FPTaylor is not affected by this problem affecting interval analysis. So the preceding statement is conflicting/confusing.}
\adcmt{I think it appeared to be confusing. Earlier it is said FPTaylor produces tight results compared to the other mentioned tools. The simplification issue for interval based solver for the optimizer still exists, that being a separate issue that using interval analysis for error propagation. I agree this part needs to be clarified upfront.}
%
\satire stresses the use of {\em simplifying
symbolic expressions} to reduce the individual occurrence of a variable
term. Here each symbolic expression is comprised 
of unique symbols representing an input variables or an abstracted node(as a free variable) such that each variable has an associated incoming error term and a numeric interval.  
%
\skcmt{do you mean repeated occurrence of a variable?
Also ``variable term'' is not defined thus far.}
%
We refer to this process as {\em canonicalization} or {\em
simplification}.
%
\skcmt{Given an idea of canonicalization.
Not good to leave it as a magic sauce.
Following sentence in unclear. Not sure how to improve it.}
\adcmt{Will add this in final intro, or Professor is going to add this
as part of his reorg we discussed earlier}
%
Feeding the optimizer with the synthesized expressions optimized for
preserving correlation (through canonicalization) aids better
convergence results for \satire.
%
\adcmt{Remove highlights as points ... discuss the table}
\adcmt{Change unique features to format as contributions}
Here are some of the
highlights of \satire:


